Enhancing Video Analytics Accuracy via Real-time Automated Camera Parameter Tuning

In Video Analytics Pipelines (VAP), Analytics Units (AUs) such as object detection and face recognition running on remote servers critically rely on surveillance cameras to capture high-quality video streams in order to achieve high accuracy. Modern IP cameras come with a large number of camera parameters that directly affect the quality of the video stream capture. While a few of such parameters, e.g., exposure, focus, white balance are automatically adjusted by the camera internally, the remaining ones are not. We denote such camera parameters as non-automated (NAUTO) parameters. In this paper, we first show that environmental condition changes can have significant adverse effect on the accuracy of insights from the AUs, but such adverse impact can potentially be mitigated by dynamically adjusting NAUTO camera parameters in response to changes in environmental conditions. We then present CamTuner, to our knowledge, the first framework that dynamically adapts NAUTO camera parameters to optimize the accuracy of AUs in a VAP in response to adverse changes in environmental conditions. CamTuner is based on SARSA reinforcement learning and it incorporates two novel components: a light-weight analytics quality estimator and a virtual camera that drastically speed up offline RL training. Our controlled experiments and real-world VAP deployment show that compared to a VAP using the default camera setting, CamTuner enhances VAP accuracy by detecting 15.9% additional persons and 2.6%-4.2% additional cars (without any false positives) in a large enterprise parking lot and 9.7% additional cars in a 5G smart traffic intersection scenario, which enables a new usecase of accurate and reliable automatic vehicle collision prediction (AVCP). CamTuner opens doors for new ways to significantly enhance video analytics accuracy beyond incremental improvements from refining deep-learning models.

==> face-recog-moti.tex <==
\subsection{Impact of different camera settings for different environment}
\label{subsec:different-settings-for-different-env}
As discussed in \S\ref{subsec:environ}, we see that a fixed camera setting can adversely impact the AU accuracy as the environment changes. In this section, we study the impact of different camera settings for different environmental conditions. Particularly, we study this under a simulated environmental change and under natural environmental change.

\subsubsection{Simulated environmental change}
\label{subsec:simulated-environmental-change}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[width=1.6 in]{figs/recall_day_excel_2.png}
    \caption{DAY}
    \label{fig:recall_day}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[width=1.6 in]{figs/recall_night_excel_2.png}
    \caption{NIGHT}
    \label{fig:recall_night}
\end{subfigure}
 \caption{Parameter tuning impact for Face-recognition AU.}
  \label{fig:recall-phy}
 \vspace{-0.3in}
\end{figure}
For simulated environmental change, we use two sources of light in our lab. One of them is always kept \emph{ON}, while the other light source is manually turned {ON} or {OFF} to simulate DAY and NIGHT environmental conditions, respectively. We place face cutouts of 10 unique individuals in front of the camera as a fixed static scene and evaluate the performance of the most accurate face-recognition AU (Neoface-v3~\cite{NIST}\footnote{This face-recognition AU is ranked first in the world in the most recent face-recognition technology benchmarking by NIST.}) for multiple face matching thresholds across various camera settings for the {DAY} and {NIGHT} environmental conditions. 

\cut{
We replay a single static scene in front of camera and evaluate the performance of the most accurate face-recognition AU (Neoface-v3~\cite{NIST}\footnote{This face-recognition AU is ranked first in the world in the most recent face-recognition technology benchmarking by NIST.}) on the capture under different camera settings. We place face cutouts of 10 unique individuals in front of the camera as a fixed static scene and run the face recognition pipeline for various camera settings and for different face matching thresholds. We rerun this experiment for two environmental conditions \ie {DAY} and {NIGHT} conditions in our lab. Since this face-recognition AU has high precision despite of environment changes, we focus on measuring Recall, \ie true-positive rate.
}

We compare AU results under the manufacturer-provided ``Default" camera settings and ``Best'' settings for the four camera parameters.
To find the ``Best'' settings, we 
change the four camera parameters to find the setting that gives the highest Recall value.
Specifically, we vary each parameter from 0 to 100 in steps of 10 and capture the frame for each camera setting. This gives us $\approx$14.6K (11$^4$) frames 
for each condition. Changing one camera setting 
through the VAPIX API takes about 200ms, and in total it took about \emph{7 hours} to capture and process the frames for each condition. 

~\figref{fig:recall_day} shows the Recall for the {DAY} condition
for various thresholds and ~\figref{fig:recall_night} shows the Recall
for the NIGHT condition for various thresholds.
%
We see that under the ``Default''
settings, the Recall for the {DAY} condition goes down at higher thresholds,
indicating that some faces were not recognized, whereas for
the {NIGHT} condition, the Recall remains constant at a low value for
all thresholds, indicating that some faces were not being recognized
regardless of the face matching thresholds.
%
In contrast, when we changed the camera parameters for both conditions to the ``Best" settings, the AU achieves the highest Recall (100\%), confirming that all the faces are correctly recognized. The ``Best" settings for {DAY} condition is different from the ``Best" setting for {NIGHT} condition (\textcolor{blue}{provide parameter values if we have}), indicating that indeed different camera settings are required for different environmental conditions.

%These results show that it is indeed possible to improve AU accuracy by adjusting the four camera parameters.

%\vspace{-0.1in}

%define virtual knobs and impacts
%This effectuates the need for camera parameter adaptation for various environmental changes.

%\subsubsection{Natural environmental change}
%\label{subsec:natural-environmental-change}

==> motivation_old.tex <==
\section{Motivation}
\label{section:motivation}
\cut{
Some of the questions that we set forth to answer are: (1) Does change in camera settings have any effect on the accuracy of AU ? (discussed in \S\ref{subsec:impactofsettings}) (2) Does change in environmental conditions have any effect on the accuracy of AU ? (discussed in \S\ref{subsec:environ}) (3) For a given deployment, is there a fixed static camera setting that works well for different environmental conditions ? (discussed in \S\ref{subsec:different-settings-for-different-env}) and (4) Is post-capture image processing enough to improve AU accuracy ? (discussed in \S\ref{subsec:notrnough})
}
%\cut{
We motivate the need for automatic, dynamic camera setting 
by experimentally showing the impact of environmental changes on AU accuracy when static and fixed camera settings are used, and 
the impact of dynamic camera parameter settings on AU accuracy 
under the same environmental conditions. In addition, we also motivate the need for automatic, dynamic tuning of camera settings by experimentally showing that post-capture image transformations are not enough and they do not achieve the same high accuracy that is possible by directly tuning the camera settings.
%}

\subsection{Impact of Environment Change on AU accuracy}
\label{subsec:environ}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.25 in]{figs/fd-performance.png}
    \caption{Face detection}
    \label{fig:daylong_face_det}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.25 in]{figs/person-performance.png}
    \caption{Person detection}
    \label{fig:daylong_person_det}
\end{subfigure}
 \caption{AU accuracy variation in a day and impact of camera settings.}
  \label{fig:face_person_env}
 %\vspace{-0.35in}
\end{figure}

\cut{
Environmental conditions change over time, and these changes affect
the quality of images and videos retrieved from a surveillance camera. 
}

Environmental changes happen for at least three reasons.
First, such changes can be induced due to the change of
the Sun's movement throughout a day, \eg sunrise and sunset.
Second, they can be triggered by 
% changes in a longer time scale than a day
% due to dynamic change in sun position, various 
changes in weather conditions, \eg rain, fog, and snow.
Third, even for the same weather condition at exactly the same
time of the day, the videos captured by the cameras at different 
deployment sites (\eg parking lot, factory, shopping mall, and airport)
can have diverse content and ambient lighting conditions.

To illustrate the impact of environmental changes on image quality, and
consequently on the accuracy of AUs, we experimentally measure the
accuracy of two popular AUs (face detection and person detection)
throughout a 24-hour (one-day) period.  Since there are
no publicly available video datasets that capture the environmental
variations in a day or a week by using the same camera (at the same location), we use
several proprietary videos provided by our customers that is captured with fixed default camera setting. These videos were 
captured outside airports and baseball stadiums by stationary surveillance cameras, 
\cut{the field of view (FoV) was fixed for the entire duration of video capture,}
and we have
labeled ground-truth information for several analytics tasks
including face detection and person detection.

We use RetinaNet~\cite{deng2019retinaface} for face detection and
EfficientDet-v8~\cite{tan2020efficientdet} for person detection. 
\cut{In both
cases, we compare the analytics results with the ground truth
information to measure the accuracy of insights from the AUs.
}
We compute the mean Average Precision (mAP) by using pycocotools~\cite{pycoco}. \figref{fig:daylong_face_det} shows that the average mAP values for the
face detection AU during four different time periods of the day
(morning 8AM - 10AM, noon 12PM - 2PM, afternoon 3PM -
  5PM, and evening 6PM - 8PM), and with the default camera parameter
settings, can vary by up to 40\% as the day progresses (blue bars).
Similarly, \figref{fig:daylong_person_det} shows that the average mAP
values for the person detection AU (with default camera parameter
settings) can vary by up to 38\% during the four time periods.
These results show that changes in environmental
conditions can adversely affect the quality of the frames retrieved from the
camera, and consequently adversely impact the accuracy of the insights that are
derived from the video data. 


%talk about two mitigation scheme
This AU performance degradation due to environment changes can be mitigated either directly tuning the real camera parameters before the capture or we can apply some postprocessing techniques on the captured scene. Next, we will show how different camera parameter settings can affect the AU accuracy differently and selecting a better camera parameter setting can improve the AU performance. Furthermore, we will observe how this choice of better camera parameter setting change with environment. 

\subsection{Impact of Camera Settings on AU accuracy}
\label{subsec:impactofsettings}

%To illustrate the impact of camera settings on AU accuracy, 
To study the impact of camera settings on AU accuracy, we consider four popular parameters that are common to almost all
cameras: {\em brightness, contrast, color-saturation} (also known as
colorfulness), and {\em sharpness}. 
%Our experiments are designed to work with scenes captured with real cameras as well as with pre-recorded videos from public datasets.

%   We note that other
%   camera parameters can also be dynamically tuned using the $\approach$
%   system. 

\begin{figure}[tp]
   \centering \includegraphics[width=0.99\linewidth]{figs/manual-camera-tuning.png} \caption{Manual camera tuning} 
   %\vspace{-0.1in}
\label{fig:system_with_human}
   \vspace{-0.2in}
\end{figure}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[width=1.6 in]{figs/cardet_left_right.pdf}
    \caption{Car Detection}
    \label{fig:cardet_improv}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[width=1.6 in]{figs/persondet_left_right.pdf}
    %\includegraphics[width=1.6 in]{figs/persondet_left_right_1.PNG}
    \caption{Person Detection}
    \label{fig:persondet_improv}
\end{subfigure}
 \caption{Impact of Camera Settings on object detection}
  \label{fig:left_right_obj}
 %\vspace{-0.3in}
\end{figure}

%show two images (side-by-side)

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/left_right_frame_266_2.PNG}
    \vspace{-0.1in}
    %\caption{Processing pipeline within a camera as part
%of a \emph{VAP}.}
    \caption{Same scene with different camera settings}
    \label{fig:left_right_cap}
%\vspace{-0.3in}
\end{figure}
 
{\bf Methodolody:}
Analyzing the impact of camera settings on video analytics is a significant challenge: it requires applying
different camera parameter settings to the same input scene and
measuring the resulting accuracy of insights from an AU.
The straight-forward approach is to use multiple cameras with different
camera parameter settings to record the same input scene. However,
this approach is impractical as there are thousands of different
combinations of even just the four camera parameters we consider.  To
overcome the challenge, we proceed with the following workaround.  


\cut{
(a) For a given environmental condition, there are thousands of camera parameter settings to choose from and (b) It will take forever to wait for different environmental conditions to occur and analyze the impact on those environmental conditions.
}

\cut{
\textbf{Methodology:}
First, we will show the impact of camera settings on a stationary scene
with a real camera.  
{Second, we apply post-capture image transformation on 
pre-recorded video snippets from public datasets to analyze the equivalent 
impact of different camera settings on those video
snippets, \ie groups of frames.}
}

\cut{
Second, we develop {\em virtual camera knobs}
which are digital equivalents of camera parameters, and then use
virtual knobs to analyze the impact of camera settings on small video
snippets, \ie groups of frames.
}

\subsubsection{Working with Real camera:}
\label{subsubsec:real-cameras}
% To test the impact of different camera parameter settings on the same scene, we replay the same scene and rerun the camera capture under different camera settings. 
%On one of the cameras, we keep the "default" manufacture-set camera settings, while on the other one we directly "modify" the camera settings manually, as shown in \figref{fig:system_with_human}.
{\bf Object detection VAP:} For experiments with real camera, we use Axis Q3505 MK II Network camera to capture (at 10 FPS) the same real-world scene.  We enact the exact same scene for different camera settings and compare the accuracy of the AU for "default" and several "modified" settings. In our scene, we have two people who walk from the camera towards a parked car, each of them then start driving separate cars in a loop within the parking lot, then park the car in the same parking spot and walk back towards the camera. This entire sequence of steps takes around 2 minutes and we repeat these exact steps over and over again for 26 different camera settings (including "default" setting). These experiments are conducted immediately one after another in quick succession to minimize the effect of environmental change.

The AU we consider in this experiment is object detection AU, which detects cars and persons in the scene. Specifically, we use Efficientdet~\cite{tan2020efficientdet} object detector across all the scenes captured under various camera settings. An illustration of the scene is shown in \figref{fig:left_right_cap} with two side-by-side frames, where the right one is with "default" camera setting while the left one is with "modified" camera setting. Here, AU can accurately detect two persons and two cars on the frame with modified camera setting while from the camera capture under default setting, AU can only able to detect one car. We observe that the accuracy of the AU varies across different camera settings and \figref{fig:left_right_obj} shows the \textit{cumulative sum} of true-positive car and person detection count~\footnote{True-positive object detection count implies that detector correctly predicts the object label and the IoU between the detected and ground-truth bounding box is more than 0.7.} for "Default Setting" and the "Modified Setting", which gives the highest accuracy among the 25 different camera settings. We see that in the "Modified Setting", there are 1890 more cars and 96 more persons correctly detected across 1300 frames.

\begin{table}[tb]
\begin{center}
\vspace{-0.15in}
\caption{Different settings for different environment.}
\label{tab:diff-env-settings}
{
\small
\begin{tabular}{|c|c|}
    \hline
    Environment & Optimal Camera Setting\\
    (Time-of-day) & [brightness, contrast, color, sharpness]\\
    \hline
    Dawn & {[80,75,50,75]}  \\
    \hline
   Morning & [30,30,50,50]  \\
    \hline
     Evening & [90,90,50,50]\\
    \hline
\end{tabular}
}
\end{center}
\vspace{-0.2in}
\end{table}
We repeat the experiment for three different times of the day \ie \textit{dawn}, \textit{Morning} and \textit{Evening} and enact the same scene across different camera settings. By repeating the experiment at different times of the day, due to varying sunlight, we get natural change in environmental conditions. ~\tabref{tab:diff-env-settings} shows that the camera setting that provides highest AU accuracy is not same as the manufacturer-provided default setting and it varies for different times of the day (\ie different environmental conditions).

%To see the impact of different camera settings on a dynamic scene, we collected multiple 2.5 minutes video snippets. Under different captures, the input dynamic scene is kept almost same as a parking lot scenario where same two persons are walking close to the parked cars then driving their cars away. Before each capture, we manually change the four camera parameters.

%We use  Efficientdet~\cite{tan2020efficientdet} object detector to detect cars and persons from the captured video snippet. We then plot the \textit{cumulative sum} of true-positive car and person detection count~\footnote{True-positive object detection count implies that detector correctly predicts the object label and the IoU between the detected and ground-truth bounding box is more than 0.7.} over the entire snippet length, shown in~\figref{fig:left_right_obj}.

%~\figref{fig:left_right_obj} shows that two different camera parameter settings result in disparate object detector performances while the object detector AU can successfully detect 1890 more cars and 96 more persons across 1300 frames captured using a modified camera setting (\ie not the default one) than under default setting. To illustrate this difference, we have shown a sample frame captured under modified and default setting in~\figref{fig:left_right_cap}. Here, AU can accurately detect two persons and two cars on the frame with modified camera setting while from the camera capture under default setting, AU can only able to detect one car. Thus, video streams (\ie group of dynamic scenes) captured under same environment with different camera parameters provide different analytics accuracy (\ie true-positive detections) and default camera setting doesn't always provide the optimal AU performance.

%static scene
{\bf Face-recognition VAP:} We place face cutouts of 10 unique individuals in front of the camera as a fixed static scene and evaluate the performance of the most accurate face-recognition AU (Neoface-v3~\cite{NIST}\footnote{This face-recognition AU is ranked first in the world in the most recent face-recognition technology benchmarking by NIST.}) for various camera settings and for different face matching thresholds.  Since this face-recognition AU has high precision despite of environment changes, we focus on measuring Recall, \ie true-positive rate.

We rerun this experiment for two environmental conditions \ie {DAY} and {NIGHT} conditions in our lab. To simulate these environmental conditions, we use two sources of light in our lab. One of them is always kept \emph{ON}, while the other light source is manually turned {ON} or {OFF} to simulate DAY and NIGHT environmental conditions, respectively.

We compare AU results under the manufacturer-provided ``Default" camera settings and ``Best'' settings for the four camera parameters.
To find the ``Best'' settings, we 
change the four camera parameters to find the setting that gives the highest Recall value.
Specifically, we vary each parameter from 0 to 100 in steps of 10 and capture the frame for each camera setting. This gives us $\approx$14.6K (11$^4$) frames 
for each condition. Changing one camera setting 
through the VAPIX API takes about 200ms, and in total it took about \emph{7 hours} to capture and process the frames for each condition. 

~\figref{fig:recall_day} shows the Recall for the {DAY} condition
for various thresholds and ~\figref{fig:recall_night} shows the Recall
for the NIGHT condition for various thresholds.
%
We see that under the ``Default''
settings, the Recall for the {DAY} condition goes down at higher thresholds,
indicating that some faces were not recognized, whereas for
the {NIGHT} condition, the Recall remains constant at a low value for
all thresholds, indicating that some faces were not being recognized
regardless of the face matching thresholds.
%
In contrast, when we changed the camera parameters for both conditions to the ``Best" settings, the AU achieves the highest Recall (100\%), confirming that all the faces are correctly recognized. The ``Best" settings for {DAY} condition is different from the ``Best" setting for {NIGHT} condition (\textcolor{blue}{provide parameter values if we have}), indicating that indeed different camera settings are required for different environmental conditions.

\if 0
\subsubsection{Pre-recorded videos:} 

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/hmdb51_face.pdf}
    \caption{Face detection}
    \label{fig:hmdb_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/hmdb51_person.pdf}
    \caption{Person detection}
    \label{fig:hmdb51_person}
\end{subfigure}
\caption{Distribution of best \emph{transformation tuple} for two AUs on \emph{HMDB} video snippets.}
\label{fig:hmdb51}
 \vspace{-0.1in}
\end{figure}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/olympics_face.pdf}
    \caption{Face detection}
    \label{fig:olympics_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/olympics_person.pdf}
    \caption{Person detection}
    \label{fig:olympics_person}
\end{subfigure}
\caption{Distribution of best \emph{transformation tuple} for two AUs on \emph{Olympics} video snippets.}
\label{fig:olympics}
 %\vspace{-0.2in}
\end{figure}

\begin{table}[tb]
\begin{center}
\vspace{-0.15in}
\caption{Impact of camera-equivalent settings}
\label{tab:best-video-conf}
{
\small
\begin{tabular}{||c|c||c|c|c|}
    \hline
    Video-Dataset & AU & \multicolumn{2}{c|}{mAP}\\
    & & \multicolumn{2}{c|}{improvement}\\
    \cline{3-4}
    & & Max & Mean \\
    \hline
    \multirow{2}{*}{Olympics} & Face Detection  & 19.23 & 1.68  \\
    \cline{2-4}
    & Person Detection & 40.38 & 8.38 \\
    \hline
    \multirow{2}{*}{HMDB} & Face Detection  & 18.75 & 4.22  \\
    \cline{2-4}
    & Person Detection & 57.59 & 12.63 \\
    \hline
\end{tabular}
}
\end{center}
%\vspace{-0.1in}
\end{table}

The pre-recorded videos from public datasets are already captured with certain camera parameter settings, and hence we do not have the opportunity to change the real camera settings and observe their impact. As an approximation, we apply different values of brightness, contrast, color-saturation and sharpness to these pre-recorded videos using several image transformation algorithms in the Python Imaging Library ({PIL})~\cite{pil}, and then observe the impact of such transformation (camera-equivalent settings) on accuracy of AU insights.

We consider 19 video snippets from the HMDB dataset~\cite{Kuehne11}
and 11 video snippets from the Olympics
dataset~\cite{niebles2010modeling}. Using cvat-tool~\cite{cvat}, we
manually annotated the face and person bounding boxes to form our ground truth. Each video-snippet contains no more than a few hundred frames.
%, and the environmental conditions vary across the video snippets {due to change in video capture locations}
We determine a single best tuple of
those four transformations for each video, \ie one that results in the highest analytical quality for that video.
%
\figref{fig:hmdb51} and \figref{fig:olympics} show the distribution of the best transformation tuples for the videos in the two datasets, respectively. We see that with a few exceptions, the best transformation tuples for different videos in a dataset do not
cluster, suggesting that different camera settings are required for different videos.
%any fixed real camera parameter settings will
%not be ideal for different environmental conditions or analytics
%tasks.  
\tabref{tab:best-video-conf} shows the maximum and average
analytical quality improvement achieved after transforming each
video-snippet as per their best transformation tuple. We observe 
up to 58\% improvement in accuracy of insights when
appropriate transformations
  or equivalent camera settings 
are applied.


%    We note that by varying the four parameters, we observe a 6.1-15.7 mAP
%    improvement for face detection AU performance on day-long video
%    segments (\figref{fig:daylong_face_det}). Similarly for the person
%    detection AU, which tries to detect the whole person rather than just
%    the face, we observe a mAP improvement of 4.9-9.7
%    (\figref{fig:daylong_person_det}). 

\cut{
Finally, we applied the above process of searching for the best camera settings
to 1-per-second sampled frames in the day-long video in \S\ref{subsec:environ}.
The green bars in \figref{fig:daylong_face_det}
and \figref{fig:daylong_person_det}
show that for face detection, the average mAP values for
the optimal settings are 6.1\% -- 15.7\% higher than for
the default settings, and for person detection the average mAP values 
under optimal settings are 4.9\% -- 9.7\% higher than 
under the default settings.
%
These results suggest that the impact of environment 
on the accuracy of AUs can be remedied
by tuning the four camera parameters to improve the image capture process.
}

\cut{
Input scenes seen by the camera are dynamic and continuously changing. While we can replay single static scene numerous times in a controlled setup but replaying a group of dynamic scenes in real world is only possible for a finite number of time \ie within a short time duration. Thus we can only get best setting among those finite settings. To overcome this limitation, we work on pre-recorded videos which can be replayed numerous times. 
}

\vspace{-0.1in}
\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-0.15in}
\if 0
\subsection{Impact of different camera settings for different environment}
\label{subsec:different-settings-for-different-env}
As discussed in \S\ref{subsec:environ}, we see that a fixed camera setting can adversely impact the AU accuracy as the environment changes. In this section, we study the impact of different camera settings for different environmental conditions. Particularly, we study this under a simulated environmental change and under natural environmental change.

\subsubsection{Simulated environmental change}
\label{subsec:simulated-environmental-change}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[width=1.6 in]{figs/recall_day_excel_2.png}
    \caption{DAY}
    \label{fig:recall_day}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[width=1.6 in]{figs/recall_night_excel_2.png}
    \caption{NIGHT}
    \label{fig:recall_night}
\end{subfigure}
 \caption{Parameter tuning impact for Face-recognition AU.}
  \label{fig:recall-phy}
 \vspace{-0.3in}
\end{figure}
For simulated environmental change, we use two sources of light in our lab. One of them is always kept \emph{ON}, while the other light source is manually turned {ON} or {OFF} to simulate DAY and NIGHT environmental conditions, respectively. We place face cutouts of 10 unique individuals in front of the camera as a fixed static scene and evaluate the performance of the most accurate face-recognition AU (Neoface-v3~\cite{NIST}\footnote{This face-recognition AU is ranked first in the world in the most recent face-recognition technology benchmarking by NIST.}) for multiple face matching thresholds across various camera settings for the {DAY} and {NIGHT} environmental conditions. 

\cut{
We replay a single static scene in front of camera and evaluate the performance of the most accurate face-recognition AU (Neoface-v3~\cite{NIST}\footnote{This face-recognition AU is ranked first in the world in the most recent face-recognition technology benchmarking by NIST.}) on the capture under different camera settings. We place face cutouts of 10 unique individuals in front of the camera as a fixed static scene and run the face recognition pipeline for various camera settings and for different face matching thresholds. We rerun this experiment for two environmental conditions \ie {DAY} and {NIGHT} conditions in our lab. Since this face-recognition AU has high precision despite of environment changes, we focus on measuring Recall, \ie true-positive rate.
}

We compare AU results under the manufacturer-provided ``Default" camera settings and ``Best'' settings for the four camera parameters.
To find the ``Best'' settings, we 
change the four camera parameters to find the setting that gives the highest Recall value.
Specifically, we vary each parameter from 0 to 100 in steps of 10 and capture the frame for each camera setting. This gives us $\approx$14.6K (11$^4$) frames 
for each condition. Changing one camera setting 
through the VAPIX API takes about 200ms, and in total it took about \emph{7 hours} to capture and process the frames for each condition. 

~\figref{fig:recall_day} shows the Recall for the {DAY} condition
for various thresholds and ~\figref{fig:recall_night} shows the Recall
for the NIGHT condition for various thresholds.
%
We see that under the ``Default''
settings, the Recall for the {DAY} condition goes down at higher thresholds,
indicating that some faces were not recognized, whereas for
the {NIGHT} condition, the Recall remains constant at a low value for
all thresholds, indicating that some faces were not being recognized
regardless of the face matching thresholds.
%
In contrast, when we changed the camera parameters for both conditions to the ``Best" settings, the AU achieves the highest Recall (100\%), confirming that all the faces are correctly recognized. The ``Best" settings for {DAY} condition is different from the ``Best" setting for {NIGHT} condition (\textcolor{blue}{provide parameter values if we have}), indicating that indeed different camera settings are required for different environmental conditions.

%These results show that it is indeed possible to improve AU accuracy by adjusting the four camera parameters.

%\vspace{-0.1in}

%define virtual knobs and impacts
%This effectuates the need for camera parameter adaptation for various environmental changes.

%\subsubsection{Natural environmental change}
%\label{subsec:natural-environmental-change}
\fi

\subsection{Impact of post-capture image processing} 
\label{subsec:notrnough}


Finally, we applied the above process of searching for the best camera settings
to 1-per-second sampled frames in the day-long video in \S\ref{subsec:environ}.
The green bars in \figref{fig:daylong_face_det}
and \figref{fig:daylong_person_det}
show that for face detection, the average mAP values for
the optimal settings are 6.1\% -- 15.7\% higher than for
the default settings, and for person detection the average mAP values 
under optimal settings are 4.9\% -- 9.7\% higher than 
under the default settings.
%
These results suggest that the impact of environment 
on the accuracy of AUs can be remedied
by tuning the four camera parameters to improve the image capture process.

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_1_excel_1.png}
    \caption{Suboptimal Setting-1 (S1)}
    \label{fig:recall_night_1}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_2_excel_1.png}
    \caption{Suboptimal Setting-2 (S2)}
    \label{fig:recall_night_2}
\end{subfigure}
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_3_excel_1.png}
    \caption{Suboptimal Setting-3 (S3)}
    \label{fig:recall_night_3}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_4_excel_1.png}
    \caption{Suboptimal Setting-4 (S4)}
    \label{fig:recall_night_4}
\end{subfigure}
 \caption{{Parameter tuning} vs. \textit{postprocessing} for {NIGHT}.}
  \label{fig:param-tune-vs-postprocess}
 %\vspace{-0.35in}
\end{figure}

\cut{
It is important to note that modifying camera parameters to capture a
better image or video feed is fundamentally different from applying transformations
to the frames already retrieved from the camera.
In particular, if the image
captured by the camera is sufficiently poor due to sub-optimal camera
settings, no further transformations of the video stream from the
camera can improve the accuracy of analytics. 

%
To see this, we repeated the same face-recognition AU experiment with a
real camera in \S\ref{subsec:simulated-environmental-change},
by intentionally
changing the default camera parameters to specific sub-optimal settings
denoted by S1, S2, S3 and S4 and measured the Recall for face
recognition AU as before. 
In these settings, the frames from the
camera are of poor quality and 
% we show 
the Recall for various
thresholds are quite low for all settings. Then, we apply
digital transformation on these  and note the
highest Recall value that we can obtain. 
}

To study the impact of post-capture image processing, we use the experimental setup discussed in \S\ref{subsec:simulated-environmental-change} for {DAY} condition and intentionally change the camera settings to specific sub-optimal settings
denoted by S1, S2, S3 and S4 and measured the Recall for face
recognition AU as before. In these settings, the frames from the
camera are of poor quality and the Recall for various
thresholds are quite low for all settings. Then, we apply
digital transformation on these and note the
highest Recall value that we can obtain.

~\figref{fig:param-tune-vs-postprocess} shows the results of actual camera parameter tuning and post-capture transformations.  We see
that for each of the four sub-optimal camera settings, post-processing
improved the Recall compared to the original video, but the Recall is
still quite low. In contrast, if we directly change the actual
camera parameters, shown as ``Best setting", then we are able to
achieve the highest possible Recall (\ie 100\%). 

This shows that modifying camera parameters to capture a
better image or video feed is fundamentally different from applying transformations to the frames already retrieved from the camera.
In particular, if the image captured by the camera is sufficiently poor due to sub-optimal camera settings, no further transformations of the video stream from the camera can improve the accuracy of analytics. 

\cut{
 This is because, due to the sub-optimal camera
settings, the frames from the camera do not have adequate information
about the scene being captured.}

%    Since we already achieve the
%    highest possible Recall value, applying further digital transformation
%    on this will not help any further. 
\cut{
This result shows that modifying camera
parameters is fundamentally different from applying transformations to
the frames retrieved from the camera.
}

\cut{
In summary, 
environmental changes can result in low-quality image acquisition, which in
turn result in poor analytics accuracy. Tuning the camera parameter
settings during capture can provide improvement in accuracy of
AUs, but such camera parameter
tuning is hard for a human to do manually because the best
parameter combination will vary with location of the camera, the type of
analytics units, and the environmental conditions.
%  Humans cannot keep
% adjusting these parameters manually, 
This calls for developing methods 
that can automatically and dynamically tune camera parameters
to improve the accuracy of AUs.
}


% We discuss the challenges and our approach in designing such a system
% design in the next section.

\vspace{0.1 in}
\noindent Revisiting our initial questions at the beginning of this section, we note that (1) Changing camera parameters \emph{does} impact the accuracy of AU (2) Changes in environmental conditions \emph{do} impact AU accuracy (3) There is \emph{no} one, fixed static camera setting that works well for different environmental conditions and (4) Post-capture image processing is not enough and we \emph{do} need camera parameter changes on real camera. Thus, in order to improve AU accuracy, as the environmental conditions change, there is a need to dynamically update camera settings so as to adapt to the changing environmental conditions.


==> oldfiles/VC.tex <==
\subsection{Virtual Camera}
\label{subsec:VC}

We design a virtual camera (VC) to accelerate initial RL training by
mimicking the effect of environmental conditions and camera setting changes
on the frame capture of a real camera.
 
{\bf Definition.} 
A VC takes an input frame $f_i$ by a real camera (with default parameter settings), the target
time-of-the-day $T_j$, and current VC virtual knob setting $V_c$,
which we refer to as virtual knobs, as input,
and outputs a frame $f_o$ as if it was captured by the physical camera
at time $T_j$ with physical camera settings $P_k$ that are equivalent to $Compose(V_c, V_k)$,
\comment{where $V_k$ is virtual knob values that is solely responsible to augment the environmental effects that correspond to o a different target time $T_j$ on the input frame, $f_i$, and $V_c$ and $V_k$ are composed into new virtual knob values by 
????. Applying the composed virtual knobs to a frame is equivalent to transforming frame to different capture time provided that $V_c$ is set to default.}


%  (see \S\ref{subsec:impactofsettings}).

% VC applies transformation on the each frame and produces the final output frame.

To understand how the virtual camera works, we first introduce an important 
definition. Each frame $f_i$ output from a physical camera
possesses distinct values of brightness, contrast,
colorfulness and sharpness metrics, denoted as a {\em metric (or feature) tuple}
$K_i = <\alpha_M$, $\beta_M$, $\gamma_M$, $\zeta_M>$.
The unique metric tuple encapsulates
the environmental conditions and the default physical camera settings
when the frame was captured.
For example, at two different times of the day
and hence under two environmental conditions,
a surveillance camera using the default settings
would output two frames with different metric tuples.


%  To change these metric values to correspond to 
%  those at a different time of the day $T_j$,
%  the VC adjusts its four camera parameter settings
%  from the current settings $V_k$ to $V_{k'}$

%  $<\alpha_P$, $\beta_P$, $\gamma_P$, $\zeta_P>$. Different
%  time-of-the-day provides different metric tuple $<\alpha_M$,
%  v$\beta_M$, $\gamma_M$, $\zeta_M>$ and that mapping is stored in the
%  \emph{VC-table}.  VC design consists of two phases: (a) online phase,
%  (b) offline profiling phase,

% During runtime, to mimic different
% environmental effects observed by the real camera, virtual camera
% takes the pre-captured video frame (of time $T_1$), 

A VC derives two tables for a given physical camera deployment during an offline profiling
phase and then uses the two tables to perform its transformation in online operations.

\textbf{Online phase}: The VC transforms the input frame $f_i$ to output frame $f_o$ in five steps.
(1) It measures the current metric  tuple
$K_i = <\alpha_M$, $\beta_M$, $\gamma_M$, $\zeta_M>_{curr}$ from input frame $f_i$;
(2) It looks up the metric tuple 
$K_{o} = <\alpha_M$, $\beta_M$, $\gamma_M$, $\zeta_M>_{desired}$ 
from a Time-to-Metric table 
that corresponds to the target time of the day ($T_j$); 
%
(3) It calculates the difference between $K_i$ and $K_o$, $\delta(K_i, K_o)$;
(4) It looks up a Metric-difference-to-Virtual-knob (MDVK) table to find the virtual knobs
$V_k = <\alpha_V$, $\beta_V$, $\gamma_V$, $\zeta_V>_{applied}$ 
that corresponds to $\delta(K_i, K_o)$; 
(5) It applies the virtual knobs $Compose(V_c, V_k)$ 
to input frame $f_i$ to generate output frame $f_o$.

Since different parts of an input frame may exhibit 
varying local feature or metric values,
to improve the effectiveness of virtual knob transformation,
instead of applying the above steps directly to input frame $f_i$, 
we split it into 12 (3 $X$ 4) equal-sized tiles
as shown in \figref{fig:vc-tiles},
apply Steps 1-3 to derive virtual knobs $V_k$ for the 12 tiles,
\ie each of $K_i$, $K_o$, and $\delta(K_i, K_o)$ consists of 
12 sub-tuples corresponding to the 12 tiles, respectively.
The 12 sub tuples in $\delta(K_i, K_o)$
are looked up in the MVDK table to find 12 virtual knobs.
Finally, to ensure smoothness,
we calculate the mean of these 12 sub-tuples $V_k$,
which is applied to 
% the 12 tiles of 
input frame $f_i$.

\if 0
(2) Training SARSA RL agent on these virtually generated sample frames
that emulates different environmental conditions accelerates RL
training convergence. Since, metric tuples for different part of the
frames show different profiles as shown in ~\figref{fig:vc-profile},
each input frame of time $T_1$ is first split into 12 tiles, also
shown in~\figref{fig:vc-tiles}. Then, for each tile, current metric
tuple, $<\alpha_M$, $\beta_M$, $\gamma_M$, $\zeta_M>_{curr}^{tile}$ is
extracted. Then, for the desired time $T_2$, the corresponding
tile-specific metric tuples are obtained from VC-table (\ie\ generated
offline) $<\alpha_M$, $\beta_M$, $\gamma_M$,
$\zeta_M>_{desired}^{tile}$. The delta change between the metric tuple
at time $T_2$ and time $T_1$ is then computed. The virtual knob
setting corresponding to the closest delta change (using L1 norm
distance~\cite{l1}) is obtained from VC delta-change table (which is
also generated offline). Once the parameter setting is obtained for
each tile, a median parameter setting, $<\alpha_P$, $\beta_P$,
$\gamma_P$, $\zeta_P>_{applied}$ is computed across tiles (to
eliminate visibility of distinct tiles in the frame) and this median
parameter setting is used to render the frame for time $T_2$. Thus,
the frame at time $T_1$ is transformed by VC to a frame at time $T_2$.
\fi

%how to get the table or mapping
\textbf{Offline profiling phase}: In this phase, we construct
the two mapping tables. 
%
%   \textit{First}, to obtain a mapping between time-of-the-day and the
%   corresponding metric (\ie\ feature) values \ie\ $<\alpha_M$,
%   $\beta_M$, $\gamma_M$, $\zeta_M>$ for that time. \textit{Second}, to
%   obtain a mapping between delta change between two metric tuples and
%   the corresponding virtual knob setting \ie\ $<\alpha_P$, $\beta_P$,
%   $\gamma_P$, $\zeta_P>$. These mapping tables are used in
%   \textit{online} phase to render the frame by VC.

The first table maps a given time-of-the-day $T_j$ to the metric tuple $V_k$
which captures the distinct values of brightness, contrast,
colorfulness and sharpness metrics of frames taken
by the physical camera with the default settings at time $T_j$.
%
We generate the table to cover the full 24-hour period
with a granularity of 15 minutes, \ie the table has one
mapping for every 15 minutes, for a total of 96 mappings.
%
To construct the table, we use a full 24-hour long video and break it
into 15-minute video snippets.
% , and thus we have 3 video snippets per 15-minute interval. 
%
We extract the frames from the video snipet for each 15-minute
interval $T_j$. We divide each frame into 12 tiles, obtain the
corresponding metric tuple for each tile, and compute the mean metric
tuple for the corresponding tiles in all frames in the 15-minute
interval as the metric tuple for that tile,
and the list of tuples for all 12 tiles form the entry 
for time $T_j$ in the table, as shown in~\figref{fig:vc-table}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The second table maps the difference between two metric tuples $K_i$
and $K_o$, $\delta(K_i, K_o)$,
to the corresponding virtual knob setting $V_k$; virtual
knobs $V_k$ would effectively transform a frame captured by the
physical camera with metric tuple $K_i$ to become a frame captured by
the physical camera for the same scene with metric tuple $K_o$.
%
We note since each camer setting can take 11 values, from 0 to 100 with
increments of 10, the total number of possible difference between any two metric tuples
is 14K ($11^4$).
%
We contruct the entries for the table backwords as follows.
(1) We select a random frame from each 15-minute interval
% \ie\ same granularity as VC-table) 
to form a collection of 96 frames with varying environmental conditions,
\ie corresponding to different time-of-the-day.
%  Again, for each of these frames, we consider separate tiles (12 per
%  frame) and for each tile, we extract the metric tuple.
(2) For each possible virtual knob setting $V_j$, 
we transform the 96 frames into 96 virtual frames. We then obtain the delta
metric tuples between each pair of original and 
transformed frames, caculate the median
of the 96 delta metric tuples, $\delta_j$, and store the pair of 
$<\delta_j, V_j>$ in the table.
(3) We repeat above the process for all possible virtual knob settings
(14K in total) 
to populate the table, as shown in~\figref{fig:delta-to-config}.
%    We generate all combinations of the possible virtual knob settings
%    that correspond to real camera parameter settings, and for each of
%    those configurations - we render the frame using the specific virtual
%    knob setting, extract $<\alpha_M$, $\beta_M$, $\gamma_M$,
%    $\zeta_M>_{render}$ on each rendered frame and then compute the delta
%    change between the original and rendered frame for each of the metric
%    tuple.
%
%  This forms a mapping between the delta change and the
%  corresponding VC parameters. By repeating the same process for all
%  frames, we have such mapping for each of the randomly selected frames
%  and for each tile. 
Finally, at runtime when the table is used by the VC, if 
the entry for a given delta metric tuple $\delta_i$ is empty,
we return the entry whose delta metic tuple $\delta_j$ is closest
to $\delta_i$ using L1-norm.
%   Lastly, we combine the delta values across all
%    frames by taking the median and generate a table, called VC
%   delta-change table, consisting of mapping between the delta change and
%   corresponding virtual configuration value, for each tile, 


\begin{figure}[tp]
 \centering
    \includegraphics[width=0.7\linewidth]{figs/vc-tiles.png}
    \caption{Tiled representation of a captured frame}
    \label{fig:vc-tiles}
\end{figure}


 \begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_bright_part_1.pdf}
    \caption{Brightness}
    \label{fig:vc-bright}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_contrast_part_1.pdf}
    \caption{Contrast}
    \label{fig:vc-contrast}
\end{subfigure}
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_color_part_1.pdf}
    \caption{Color-Saturation}
    \label{fig:vc-color}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_sharp_part_1.pdf}
    \caption{Sharpness}
    \label{fig:vc-sharp}
\end{subfigure}
 \caption{Day-long feature profiles for different tiles}
  \label{fig:vc-profile}
 %\vspace{-0.2in}
\end{figure}

%\if 0
\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=0.9 in]{figs/vc-table-1.PNG}
    \caption{VC Table}
    \label{fig:vc-table}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=0.9 in]{figs/delta-table-1.PNG}
    \caption{Delta-to-Configs Table}
    \label{fig:delta-to-config}
\end{subfigure}
 \caption{Offline Generated Tables}
  \label{fig:vc-tables}
 %\vspace{-0.2in}
\end{figure}
%\fi


\subsection{Integrating VC with the RL engine}
\label{subsec:vc-sim}

%  Fig. \ref{fig:eval_setup} shows $\approach$ system design with VC,
%  where the RL agent changes the virtual knobs and learns much quickly
%  using such a setup with VC.
A VC can be used to speed up initial RL training 
upon camera deployment at a new surveillance site 
which enhances the overall SARSA training convergence 
for two reaons:
%  While training the RL module, as shown in~\figref{fig:eval_setup},
%  during \emph{initial fast exploration phase} RL agent uses the APIs
%  exposed by VC to change the virtual knob values and learns much
%  quickly, as 
(1) it can augment each frame in a training video, \eg recorded in an hour
in the morning, with many different frames corresponding
to different environmental conditions, \eg throughout a day, and thus
omit the need to wait for video capture over a long time;
(2) the RL agent can take actions, \ie resetting virtual knob values in the VC
much faster than driving a phycial camera and hence performs 
RL exploration much faster.
% up to 300 FPS, by using more computing hardware, 
% and (3) virtual knob values can be changed instantly. 

During initial RL traniing, The RL agent drives the VC by performing
exploration as follows.
(1) It reads each frame $f_i$ from the input training video,
and repeats the following 4 steps of exploration steps for 
all time-of-the-day values $T_j$.
(2) At each exploration step $j$,
the agent which is at state $s$,
takes an action $a$ by randomly picking a new virtual knob setting
$V_j$ and reconfigures the VC with $V_j$;
(3) It invokes the VC with frame $f_i$, the next 
time-of-the-day $T_j$, and current VC parameters $V_c$ as input,
and the VC outputs frame $f_o$.
%
The measured tuple $P_j$ of 
brightness, contrast, colorfulness and sharpness metrics values
%  i.e., $<\alpha_M$, $\beta_M$, $\gamma_M$, $\zeta_M>$ 
of output frame $f_o$ 
along with the current VC virtual knobs $V_j$, 
$s_{new} = <P_j, V_j>$,
form the new state of the RL agent;
(4) It caculates the reward/penality by feeding $f_o$ into
the AU-pecific quality estimator;
(5) It updates the Q-table entry $Q(s, a)$.


\if 0
During fast initial training, each
output frame from virtual camera corresponds to a specific state of
These current virtual camera parameters
(\ie\ virtual knob setting, $<P_{RL}>$ = $<\alpha_P$, $\beta_P$,
$\gamma_P$, $\zeta_P>_{RL}$) are decided by the RL agent based on
previous output frame state. Along with virtual camera parameter
tuning, to emulate various environmental conditions, VC also attempts
to the VC parameters (\ie\ $<P_{VC}>$ = $<\alpha_P$, $\beta_P$,
$\gamma_P$, $\zeta_P>_{VC}$). During initial training, we apply a
virtual knob setting that is resulted from combining two parameter
tuples \ie\ $<P_{RL} \circ P_{VC}>$. 
\fi

The above initially trained SARSA model with VC is then deployed in the real camera for the normal operations
of \approach.
First, the epsilon value is set to low (0.1)
so that the SARSA RL agent will go through an \emph{adaptation} phase, \eg for an hour,
by performing primarily exploration.
Afterwards, the epsilon value is to set to high (0.9) so that SARSA performs primarily
exploitation using the trained model.

% After few episodes of exploration with real camera, 

%  we keep the epsilon for first few episodes to be low
%  (0.1) so that it can explore more by taking actions on the real camera
%  parameters based on environment observed at deployment site. 



%\textcolor{red}{mention about initial exploration then exploration with real camera and then final exploitation and also epsilon changes}


==> oldfiles/abstract.tex <==
\begin{abstract}
Complex sensors like video cameras include tens of configurable parameters, which can be set by end-users to customize the sensors to specific application scenarios. Although parameter settings significantly affect the quality of the sensor output, and the accuracy of insights derived from sensor data, most end-users use a fixed parameter setting because they lack the skill or understanding to appropriately configure these parameters. We propose $\approach$, which is a system to automatically, and dynamically adapt the complex sensor to changing environmental conditions. We show that by automatically, and dynamically updating the parameter settings to adjust to the changing environmental conditions near the sensor, it is possible to significantly improve the accuracy of inferred insights. 
$\approach$ includes two key components. \textit{First}, a bespoke analytics quality estimator, which is a deep-learning model to automatically and continuously estimate the quality of insights from an analytics unit as the environmental conditions around a sensor change. \textit{Second}, a reinforcement learning (RL) module, which reacts to the changes in quality (as perceived by the quality estimator), and %reinforcement learner learns a model to 
automatically adjusts the camera parameters to enhance the accuracy of insights. 

We improve the training time of the RL module by an order of magnitude by designing two virtual models to mimic the essential behavior of the camera: we design {\it virtual knobs} that can be set to different values to mimic the effects of assigning different values to the camera's configurable parameters, and we design a {\it virtual camera} model that mimics the output from a video camera at different times of the day. These virtual models significantly accelerate training because (a) frame rates from a real camera are limited to 25 to 30 fps while the virtual models enable processing rate of 300 fps, (b) we do not have to wait until the real camera sees different environmental conditions, which could take weeks or months, and (c) virtual knobs can be updated instantly, while it can take 200-500 ms to change the camera parameter settings using APIs provided by the camera-vendor. Our dynamic tuning approach results in up to 12\% improvement in the accuracy of insights from several video analytics tasks. Also, $\approach$'s sensor modelling and dynamic tuning methodology can be used to automatically, and dynamically tune other complex sensors.


%The virtual knobs model allows the application of different camera parameter settings to the same input scene (something that is not possible to do with the real camera because only one set of camera parameter values can be in effect at any given time). The virtual camera model (described in Section~\ref{alg:vc-sim}) allows re-rendering of any video sequence for different environmental conditions. This is especially useful to quickly train the reinforcement learning model because multiple versions of a video sequence with known ground truth can be quickly rendered for different environmental conditions. Again, such a re-rendering of the same video scene for different environmental conditions is not possible with a real camera.
%Furthermore, the environmental conditions around the sensors can vary considerably during the lifetime of the sensor applications, and parameter settings may have to be updated multiple times to ensure consistent, high quality sensor data and insights.
%\emph{Video analytics} has become popular but currently it is gaining even more attention in this mid COVID-19 era. Citywide ubiquitous edge-camera deployments facilitate different analytics being perfor 
%With growing deployment of video cameras throughout cities for various purposes, gaining valuable insights through video analytics still is quite challenging. 
%\emph{Video analytics} has become popular in the past decade due to advancement in computer vision algorithms, deep learning, edge computing, 5G, etc. This market has gained even more traction during this COVID-19 era because authorities are seeing value in performing analytics on video feed to handle emerging COVID-19 specific applications like limiting crowd, enforcing social distancing, contact tracing, etc. City-wide, ubiquitous edge-camera deployment enables a variety of analytics tasks to be performed on video feeds. These video feeds, however, are directly affected by the environment (which keeps changing) in which they are deployed in. Without accounting for the change and adapting to it, the accuracy of analytics tasks degrades significantly. In this paper, we propose $\approach$, which uses reinforcement learning techniques to continuously adapt to changing environmental conditions. Particularly, $\approach$ tunes specific camera parameters, so that the video feed produced by the camera is suitable for the analytics task at hand and improves its accuracy. $\approach$ is designed in such a way that it can be applied to any video analytics task and can handle any set of complex camera parameters. We study the impact of various camera settings on accuracy of several real-world video analytics applications and show that $\approach$ improves accuracy of video analytics applications by 12\%.
\end{abstract}

==> oldfiles/analysis.tex <==
\section{Impact of camera settings on AU}
We analyze the impact of camera settings on the accuracy of insights from AUs. This will require that we apply different camera parameter settings  to the same input scene, and evaluate the impact on the accuracy of insights from AUs. One option is to use multiple cameras with different camera parameter settings to record the same input scene. However, there are thousands of different combinations of just the four camera parameters that we focus on in this paper, and it is impractical to use real cameras to analyze the impact on AUs. Therefore, we propose {\it Virtual knobs}, which are digital equivalents of the camera parameters, to analyze the impact of camera parameter changes on the accuracy of insights. Section~\ref{virtual-knob} describes the design of virtual knobs. 

%To understand impact of camera settings on AUs, we have to apply different camera settings for the same input scene. As the scenes are continuously changing, to study this impact, one option is to use multiple cameras with different settings that record the same input scene. However, there are thousands (even millions) of different camera settings for just the four knobs we selected, and it is impractical to use so many cameras to record the same input scene. So, we propose a practical alternative of \emph{virtual knobs, a digital equivalent for the actual camera parameter.}


%Since there exists atleast one best-possible camera setting that can improve the AU accuracy observed under default setting, we first study how different combinations of camera parameters can impact distinct images and video-snippets captured under various environmental conditions differently.  

%\subsection{Camera-Digital Twin}
\subsection{Virtual knobs}
\label{virtual-knob}
%To understand impact of camera settings on AUs, we have to apply different camera settings for the same input scene. As the scenes are continuously changing, to study this impact, one option is to use multiple cameras with different settings that record the same input scene. However, there are thousands (even millions) of different camera settings for just the four knobs we selected, and it is impractical to use so many cameras to record the same input scene. So, we propose a practical alternative called \emph{virtual knobs, a digital equivalent for the actual camera parameter settings.}

%In order to have repeatability and consistency in our analysis, we need to be able to capture one particular scene and be able to apply different camera settings on the same scene. As the scene continues to change and a camera can have only a single settings for various knobs, it becomes imperative for us to find a digital equivalent for the actual physical settings on the camera. This digital equivalent should faithfully produce the image as if it was captured by changing the physical settings on the camera itself. We refer to this digital equivalent as \emph{virtual knob}.

%Images and video-segments in public-Datasets are already preprocessed with certain camera configurations after their capture in raw format. Augmenting various different camera settings on top of that digitally through software API requires correlation with the actual knob of the camera. 

Our goal is to design proxies for the four camera parameters. We use a camera and an image transformation algorithm in the Python Imaging Library~\cite{pil} to design the virtual knobs. 

Algorithm~\ref{alg:digital-twin} describes our method to establish a correspondence between parameter values of the image transformation algorithm (which are the virtual knobs), and camera parameter values. Establishing such a correspondence is quite useful. For example, given an image, the image transformation algorithm can be used to create many modified images (by applying different combinations of the four parameter values). Then, modified images can be processed by the analytics unit to identify a combination of values (of the four parameters) that yields the best analytical results, and this combination can be mapped back to a set of camera parameter values by using the correspondence. So, by applying the correspondence, we can determine good values for the camera parameters, and for these camera parameter values, the frames produced by the camera will result in highly accurate insights from the  analytics unit.

We determine the correspondence between the parameter values of the image transformation algorithm, and the camera parameters, as follows. We set the camera parameters to their mid-range, or as recommended by the camera manufacturer, and we capture an image {\it im}. Algorithm~\ref{alg:digital-twin} has an outer loop where we progressively change the camera parameter values (through the range of values supported by the camera vendor for each camera parameter) and generate different images $im_p$ for a static scene. For each image $im_p$, which corresponds to a particular camera parameter setting,  the inner loop determines the closest set of parameter values of the image transformation algorithm that will produce a modified image $im_d$ that has the same image quality as $im_p$. These set of parameter values of the image transformation algorithm (i.e. the virtual knobs) now correspond to the specific camera parameter settings that generated the image $im_p$.  By repeating the above procedure, we determine the correspondence between different camera parameter settings and the different parameter values of the image transformation algorithm.

We use de-facto full-reference image-quality assessment metric, structural similarity (\textit{SSIM})~\cite{ssim} to match the image quality of $im_p$ (image from camera) and $im_d$ (modified image produced by the image transformation algorithm). For example, if the SSIM value for the pair ($im_p$,  $im_d$) is higher than 0.9, then the image from the camera and the modified image from the image transformation algorithm are both of good visual quality~\cite{cuervo2015kahawai}. ~\tabref{tab:cam-twin-final} shows the range for the virtual knobs that correspond to the full range of camera parameter settings (usually, between 0 and 100).
%We use several different full-reference image-quality assessments (SSIM or structural similarity (\textit{SSIM})~\cite{ssim}, MS-SSIM or multiscale-structural similarity (\textit{MS-SSIM})~\cite{wang2003multiscale}, MSE and PSNR) to match the image quality of $im_p$ (image from camera) and $im_d$ (modified image produced by the image transformation algorithm). For example, if the SSIM value for the pair ($im_p$,  $im_d$) is higher than 0.9, then the image from the camera and the modified image from the image transformation algorithm are both of good visual quality~\cite{cuervo2015kahawai}.

%The correspondence between the virtual knobs of the image transformation algorithm, and the camera parameters, depends on the image quality assessment method. ~\tabref{tab:cam-twin} shows the range of parameter values for the image transformation algorithm (i.e. virtual knobs) that correspond to the full range of camera parameter settings (usually, between 0 and 100). We take the union of the ranges for  different image quality assessment methods as the range for the virtual knobs (the final ranges for the virtual knobs are shown in ~\tabref{tab:cam-twin-final}).


%We use the image transformation algorithm in the Python Imaging Library~\cite{pil} to design the virtual knobs. Given a frame, the image transformation algorithm can apply different combinations of values for the four parameters (brightness, contrast, color-saturation, and sharpness), and create modified versions of the input frame. Then, we apply different full-reference image-quality assessments (SSIM or structural similarity (\textit{SSIM})~\cite{ssim}, MS-SSIM or multiscale-structural similarity (\textit{MS-SSIM})~\cite{wang2003multiscale}, MSE and PSNR) to assess the image quality of the modified frame.

%Algorithm~\ref{alg:digital-twin}, we found corresponding \emph{virtual knobs} for those four camera parameters (mentioned in ~\secref{sec:cam-tuning-params}) for \emph{AXIS Q1615 Network Camera}. We search the digital range corresponding to the camera parameter range. This range helps us to find the equivalent search-space in digital domain which can also be achieved by traversing the entire camera settings space. 
%To achieve that, we find the mapping of discrete camera parameter values to corresponding virtual knob values by finding maximum similarity between frame obtained with camera parameter value and augmented frame taken under default camera setting using digital augmentation~\cite{pil}. We rely on full-reference Image-Quality assessments (i.e., FR-IQA like structural similarity (\textit{SSIM})~\cite{ssim}, multiscale-structural similarity (\textit{MS-SSIM})~\cite{wang2003multiscale}, MSE and PSNR) to determine the equivalence of camera parameter and virtual knob values.
%The corresponding knob value in digital domain is only treated as the faithful representation of a actual camera parameter value when images obtained in both domains with respective knob values provide the maximum SSIM~\cite{ssim}, which is atleast greater than 0.90~\footnote{\emph{de facto} image-quality metric, SSIM value higher than 0.90 indicates that the images obtained in digital domain well approximates the original captured frame where camera parameters are set and provides “good” visual quality~\cite{cuervo2015kahawai}}.
%The equivalent search-space in digital domain is dependent on (1) the image transformation algorithm being used to perform the mapping and (2) FR-IQA methods. These various equivalent search-space ranges in digital domain for an allowable camera parameter range (i.e., [0,100]) are listed in ~\tabref{tab:cam-twin}. 
%Finally, we take the union of these different ranges obtained for different FR-IQA methods for a particular tuning parameter as our equivalent digital search-space, also listed in ~\tabref{tab:cam-twin-final}.

\begin{algorithm}%[tp]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwFunction{FAugment}{Augment}
  \SetKwFunction{FSSIM}{SSIM}

\Input{\begin{minipage}[t]{6.5cm}%
     Virtual Knob Values $dval_{list}$;
     
     Camera Parameter Values $pval_{list}$;
   \end{minipage}
  }
  
  \caption{Camera Parameter-to-Virtual Knob Mapping}
  \label{alg:digital-twin}
    Obtain $im$ with default camera parameter value $pval_{default}$; %(i.e., 50);

    \For{p in $pval_{list}$}{
        Obtain $im_{p}$ from the camera changing camera parameter to $p$
        \For{d in $dval_{list}$}{
            $im_{d}$ $\leftarrow$ \FAugment($im$,$d$);
  
            ssim-val(d) $\leftarrow$ \FSSIM($im_{p}$,$im_{d}$)
        }
        $d_{virtual}$ $\leftarrow$ $\argmax_{d}$ ssim-val(d)
        
        \KwRet{(p,$d_{virtual}$)} 
    }
 }
\end{algorithm}
\if 0
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Tuning & \multicolumn{3}{c|}{Virtual-Knob Range}\\\cline{2-4}
    Parameter & MSE/PSNR & SSIM & MS-SSIM \\\hline
    Brightness  & [0.6,1.5] & [0.7,1.2] & [0.8,1.1]\\\hline
    Contrast & [0.6, 3.5] & [0.6, 3.6] & [0.6, 3.3] \\\hline
    Sharpness & [0.5,1.2] & [0.5,1.0] & [0.5,1.3] \\\hline
    Color-Saturation & [0.1,2.0] & [0.1,1.0] & [0.1,1.5]\\\hline
\end{tabular}
\caption{Virtual Knob Range for different IQA methods}
\label{tab:cam-twin}
 \vspace{-0.3in}
\end{table}
\fi

\if 0
\begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[MSE]{\includegraphics[width=3.8cm]{figs/twin_mse.PNG}\label{fig:twin_mse}}
 & \subfloat[SSIM]{\includegraphics[width=3.8cm]{figs/twin_ssim.PNG}\label{fig:twin_ssim}
 }
 \end{tabular}
 \end{tabularx}
 \caption{Digital Twin}
  \label{fig:digital_twin}
 \end{figure}
 \fi
 
 \begin{table}[h!]
 \centering
 \begin{tabular}{||c|c||}
 \hline
 Tuning-param & Range of \emph{virtual knob} \\ \hline
 Brightness & [0.6, 1.6] \\ \hline
 Contrast & [0.6, 3.6] \\ \hline
 Sharpness & [0.5, 1.6] \\ \hline 
 Color-Saturation & [0.1, 2.0] \\ \hline
 \end{tabular}
 \caption{Virtual Knob Ranges}
 \label{tab:cam-twin-final}
 \vspace{-0.2in}
 \end{table}
 
%With the digital equivalence, we find best virtual knob settings for any given an image or video-frame. Then, we can apply the inverse-mapping to find corresponding camera parameter setting. Thus, we can estimate what the best camera parameter settings are for a given
%input scene.
 
%\subsection{Changing One parameter at a Time}
\subsection{Impact of varying virtual knobs}
\label{sec:knob-impact}

\if 0
\subsubsection{one knob at a time}
With the equivalent range of parameters in digital domain, we next investigate how AU accuracy varies while changing one of the four parameters at a time for all the images or frames . In this section, we are looking into the best-possible impact on AU accuracy changing a single parameter once. 
%granularity is dataset and also one parameter at a time

Changing the \textit{color-saturation} impacts analytical accuracy for face detection (i.e., mAP) by 5\% for 100 randomly fivek raw-image dataset~\cite{fivek}. While varying single tuning knob, Face-recognition AU~\cite{schroff2015facenet} also recognizes 10 more images out of 1150 celebrity images randomly selected from celebA~\cite{liu2015faceattributes} dataset than the baseline~\footnote{baseline=camera parameters under deafault settings}. Liveness detection AU~\cite{wu2020uncertainty} detects whether an image is real or fake (i.e., plays significant role for cashless transactions), improves binary classification accuracy by 6.8\% while changing the \textit{contrast} tuning knob, leads to 20 more images out of 280 images from MSU-MFSD dataset~\cite{wen2015face} being correctly classified as \textit{real} or \textit{fake}. 

Variation in \textit{color-saturation} tuning knob (i.e., keeping other knobs fixed) improves the mAP by 7\% for face detection AU on proprietary night-time video. On Olympics action-dataset~\cite{niebles2010modeling} video-snippets, while varying \textit{contrast} improves the mAP of person detection AU by 9\%, mAP of face detection AU gets improved through varying the \textit{color-saturation}.
\fi

%\subsubsection{Changing all knobs simultaneously}
 %Even coarse-grained way of tuning a single parameter independently on all images present in a dataset can provide better analytical results as shown in previous section. But since, impact of each camera tuning knobs on the analytics accuracy is non-monotonic in nature and 
 
 %In this section, we study the tuning of those four virtual knobs (mentioned in ~\secref{sec:cam-tuning-params}) for each static-image and video-snippet which is captured under different environment and with different camera-settings.
 
 We analyze the impact of changing the values of virtual knobs on the accuracy of insights from the analytics units. We consider images and video snippets from popular public datasets. These images and videos were captured under different environmental conditions, and by different cameras with unknown camera settings. Our analysis (a) quantifies the possible improvement in the accuracy of insights by tuning virtual knobs, (b) demonstrates that different camera parameter settings are desirable for different environmental conditions, and (c) identifies the specific camera parameter setting that can enhance the accuracy of insights from the analytics unit.
 
  

 
 \subsubsection{Static images}
 We consider images in public datasets like  Fivek RAW dataset~\cite{fivek} and celebA~\cite{liu2015faceattributes}. These images were taken using different cameras, and under different environmental conditions. For each image, we determine the best combination of virtual knobs that results in the most improvement in accuracy of insights from the analytics units.
 
% Each image available in public-datasets (i.e., Fivek RAW dataset~\cite{fivek}, celebA~\cite{liu2015faceattributes}, 300W~\cite{sagonas2016300}) is a proxy for video snippet that would have been taken around the time the image was taken. Hence each image is captured under a different environment and using different camera settings. 
 %Hence, each image corresponds to a unique environmental condition and  camera setting. 
 %Best parameter setting at camera corresponds to the configuration that provides best analytic quality (AQ) which is specific to each AU, described as follows:

\if 0 
  \begin{algorithm}%[tp]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}

  
  \caption{Best Tuple Search for a Static Image}
  \Input{\begin{minipage}[t]{6.5cm}%
     Image $im$; 
     Analytical Unit $AU$ and corresponding Analytical Quality $AQ$;
   \end{minipage}
  }
  \Output{Find best tuple value <bright,contrast,color,sharp> that provides best $AQ$}
  \label{alg:best-tuple-search}
}
\end{algorithm}
 \fi

 \paragraph{Person and Face Detection AUs:} We use efficientdet-v0~\footnote{input-size of efficientdet-v0 closely matches with the raw image resolution while compared with other efficientdet variants.} as the person detection AU and Retinanet as the face detection AU, and perform analytics on a random subset of 100 Fivek {\it raw} images. First, we manually annotated the 100 images to detect persons and the bounding boxes for their faces using cvat-tool~\cite{cvat}. This is the ground truth.  Then, for each AU, we used Algorithm~\ref{alg:det-conf-search} to identify the best combination of virtual knobs for the AU by using a combination of mAP and true-positive IoU~\footnote{where single bounding box prediction for a object with IoU>0.5 with correct classification} as the analytical quality metric. When we use the best combination of virtual knobs for each image, and modify the image using this combination of values for the four parameters, the AU performance improves. For example, the face detection AU detects faces in \emph{39} more images when compared with face detection on the original 100 images. The distribution of the best virtual knob combination for each image is shown in ~\figref{fig:raw_AU}. Each point in the figure corresponds to an image in the subset of 100 Fivek images, and the coordinates of the point are the best virtual knob combination for the image~\footnote{We first use the virtual knob range shown in ~\tabref{tab:cam-twin-final}, but since we observed that the best configuration is towards the upper-limit of those ranges, we extended the virtual knob range to make sure we are not missing out on other possible best configuration.}. Clearly, the best combination of virtual knobs for each image are not clustered, suggesting that a single, fixed camera parameter setting is not ideal. 
 
 %shows how \emph{these best-configuration (i.e., that improves AQ) for different raw images varies over the entire virtual knob space}.
 
 %The selection of the best combination is done in a two-step process. We first determine a set of combinations, all of which result in the highest mAP. Then, we break the tie by selecting the virtual knob combination with the highest \textit{true-positive detection}~\footnote{where single bounding box prediction for a object with IoU>0.5 with correct classification} IoU jointly as analytical quality (AQ) metric. ~\figref{fig:raw_AU} shows how \emph{these best-configuration (i.e., that improves AQ) for different raw images varies over the entire virtual knob space}.
 
%We first use the parameter range shown in ~\tabref{tab:cam-twin-final}, but we observed that the best configuration is towards the upper-limit of those parameter ranges obtained through digital-twin. Hence, we extended the configuration space to make sure we are not missing out on other possible best configuration. 

%\textcolor{blue}{If this might confuse the reader, you can show with original knob space.}


%Similarly, the person detection AU has an mAP improvement of 2.8\% on average and an IoU improvement of 6.7\%. Hence, we observe higher improvement after tuning for finer-grained analytics like face detection (i.e., with more true-positive detections), while compared with person detection for same set of images.

%in the modified images. base-configuration~\footnote{base-configuration = camera parameters under default settings} where face detection AU can detect faces only in 33 images. Even for those 33 images (i.e. detected in base-configuration), best-configuration tuning improves the average true-positive IoU by 5.6\%. 


%Tuning each raw image with its best-configuration helps face detection AU to detect faces in \emph{39} more images than base-configuration~\footnote{base-configuration = camera parameters under default settings} where face detection AU can detect faces only in 33 images. Even for those 33 images (i.e. detected in base-configuration), best-configuration tuning improves the average true-positive IoU by 5.6\%.
%For person detection AU, best-configuration tuning provides mAP improvement of 2.8\% on average and an IoU improvement of 6.7\%. Hence, we observe higher improvement after tuning for finer-grained analytics like face detection (i.e., with more true-positive detections), while compared with person detection for same set of images.
 
%Face detection AU is able to detect faces in 39 more images (compared with only 33 detections under base-configuration, results in 118.18\% improvement) after tuning with best-configuration, while for person detection AU, best-configuration tuning provides mAP improvement of 2.8\% on average and an IoU improvement of 6.7\%. Hence, we observe higher improvement after tuning for finer-grained analytics like face detection, while compared with person detection for same set of images.
 
 \begin{algorithm}%[tp]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
    \SetKwFunction{FmAP}{mAP}
  \SetKwFunction{FAU}{AU}
  \SetKwFunction{FAugment}{Augment}
  
  \caption{Find Best Configuration for Detection}
  \label{alg:det-conf-search}
  \Input{\begin{minipage}[t]{6.5cm}%
     Image $im$ and ground-truth $gt$;
     Configurations $confs$
   \end{minipage}
  }
  \Output{Find conf:<bright,contrast,color,sharp> that provides best $AQ$ for detection}
  \For{$i$ in $confs$}{
    $im_{aug}$ $\leftarrow$ \FAugment($im$,$i$);
    
    $dets$ $\leftarrow$ \FAU($im_{aug}$);
    
    mAP, true-positive IoU $\leftarrow$ \FmAP($dets$, $gt$) with 0.5 iou-threshold;
}

First Sort $confs$ using corresponding mAP;

Then for same top-1 mAP $confs$ sort using true-positive IoU;

\KwRet{top-1 $conf$ from final sorted list}
}
\end{algorithm}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/raw_face.pdf}
    \caption{Face Detection}
    \label{fig:raw_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/raw_person.pdf}
    \caption{Person Detection}
    \label{fig:raw_person}
\end{subfigure}
\caption{Distribution of best configurations for different AU on \emph{fivek raw-dataset}}
\label{fig:raw_AU}
 \vspace{-0.2in}
\end{figure}
 
% \begin{figure}
%\def\tabularxcolumn#1{m{#1}}
% \begin{tabularx}{\linewidth}{@{}cXX@{}}
% \begin{tabular}{cc}
% \subfloat[face detection]{\includegraphics[width=3.8cm]{figs/raw_face.pdf}\label{fig:raw_face}}
% & \subfloat[person detection]{\includegraphics[width=3.8cm]{figs/raw_person.pdf}\label{fig:raw_person}
% }
% \end{tabular}
% \end{tabularx}
% \caption{Optimal Camera Tuning Confs on \emph{fivek raw-dataset}}
%  \label{fig:raw_AU}
% \end{figure}
 
 \paragraph{Face Recognition AU:} We use the face-recognition AU pipeline described in ~\cite{schroff2015facenet}. 
 %This AU determines if an input face image matches with any image in a pre-defined gallery of face images. 
 %Given a database of person with atleast one face-image associated to the person, the AU either recognizes the faces in the input-image as known persons (already present in the database) with a \emph{match-score}, or it classifies it as unknown. 
 We use one face image of each person in the CelebA dataset to populate the pre-defined gallery of face images, and use the remaining face images as queries. The analytical quality metric for face-recognition AU is the true-positive match-score. We use Algorithm~\ref{alg:det-conf-search}, and this quality metric, to determine the best virtual knob configuration for each person in the 300-person CelebA dataset. 
 %put the relative improvement
When we modify the query images by using their best virtual knob settings, then face-recognition AU recognizes \emph{41} more face-images correctly when compared to recognition on the original query images (faces in 256 original images are correctly recognized). Moreover, best virtual knob configuration for each query image improves the average true-positive match-score by 3.6\% (e.g., maximum AQ improvement ~ 11.6\%).
%with base-configuration, where only 256 faces are correctly recognized, Moreover, best-configuration tuning for each query image improves the average match-score (i.e., AQ) by 3.6\% (e.g., maximum AQ improvement ~ 11.6\%). Hence, best-configuration not only improves the matchScore for each image but also improves the overall recognition accuracy. 
The distribution of the best virtual knob combination for each query image is shown in ~\figref{fig:face_recog}. Again, each point in the figure corresponds to an image in the 300-person CelebA dataset, and the coordinates of the point are the best virtual knob combination for the query image. Clearly, again, the best combination of virtual knobs for each image are not clustered, suggesting that a single, fixed camera parameter setting is not ideal. 
%\emph{How the best combination of those four knobs varies for different images for face-recognition AU is shown in ~\figref{fig:face_recog}}.
 %Changing minEyeDistance configuration from 20 to 40 provides a drastic improvement in recognition with 26.05\% more images being recognized with best-configuration augmentation while compared with base-configuration. 
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/image_facerecog.pdf}
    \caption{Distribution of best configurations for face-recognition AU on \emph{CelebA}}
    \label{fig:face_recog}
     \vspace{-0.2in}
\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/image_facerecog.pdf}
    %\vspace{-0.2in}
%    \caption{Optimal Camera Tuning Confs for face-recognition AU on \emph{CelebA}}
%    \label{fig:face_recog}
    %\vspace{-0.1in}
%\end{figure}
 
 \paragraph{Facial Keypoint Detection AU:} Facial keypoint detection AU ~\cite{kazemi2014one} detects 68 facial landmarks in a face. We use images from the 300W dataset~\cite{sagonas2016300}. Analytical quality metric for this AU is the root-mean-square (RMS) distance between the predicted and actual landmarks~\footnote{low RMS distance implies better analytical quality}. If we modify each image by using its best virtual knob configuration, then the facial-keypoint detection AU detect facial landmarks in 11 more images. Also, for the 215 images where facial landmarks were detected by the AU by using the original images, the analytical quality of their corresponding, modified 215 images improved by an average of 31.1\%. This shows that camera parameter tuning generally improves the analytical quality of all images. \figref{fig:facial_kp} shows the distribution of the best combination of virtual knob values for all the images in the 300W dataset, and again, the best virtual knob configurations do not cluster. Therefore, a single, fixed camera parameter setting is not ideal.  
 %best configurations scatter throughout the configuration knob space for different images. 
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/image_facial_kp.pdf}
    \caption{Distribution of best configurations for facial-KP AU on \emph{300W}}
    \label{fig:facial_kp}
     \vspace{-0.2in}
\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/image_facial_kp.pdf}
    %\vspace{-0.2in}
%    \caption{Optimal Camera Tuning Confs for facial-KP AU on \emph{300W}}
%    \label{fig:facial_kp}
    %\vspace{-0.1in}
%\end{figure}

 
%The dispersion of the best-parameters throughout the configuration space establishes that each image taken in a different environment with a different camera setting requires different attention (i.e. different best-configurations). 

%\paragraph{Liveness Detection AU:} This AU~\cite{wu2020uncertainty} detects whether a face image is real or fake (plays significant role in anti-spoofing). \emph{AQ} for this AU is defined as the accuracy for classifying a face image as \textit{real} or \textit{fake}. Best virtual knob tuning improves this binary classification accuracy by 6.8\% which leads to 20 more images out of 280 images from MSU-MFSD dataset~\cite{wen2015face} being correctly classified as \textit{real} or \textit{fake}. Due to space constraint, we didn't show best configuration distribution plot across various images for liveness detection AU, but we observed similar scatter in best configurations for different images (i.e. representing different environment) from MSU-MFSD dataset.
 
\subsubsection{Video snippets} We analyze the impact of virtual knob settings when analytics are performed on videos. We consider 19 video snippets from HMDB dataset~\cite{Kuehne11} and 11 video snippets from Olympics dataset~\cite{niebles2010modeling}. Similar to the images case, we manually annotated the face and person bounding boxes. This is our ground truth.
Each video-snippet contains no more than a few hundred frames, and the environmental conditions for a video are largely constant. However, the environmental conditions appear to vary across the video snippets. We determine one best combination of virtual knobs for each video.  \figref{fig:hmdb51} and \figref{fig:olympics} show the distribution of the best virtual knob combinations for the 19 videos in the HMDB dataset and the 11 videos in the Olympics dataset, respectively. Again, the best virtual knob combinations for each video in a dataset do not cluster (although there are a few of them that overlap), suggesting that a fixed camera parameter setting is not ideal for different environmental conditions or analytics tasks.  

%Again, the best virtual knob combinations for each video in a dataset do not cluster, suggesting that a fixed camera parameter setting is not ideal for different environmental conditions or analytics tasks. 

%how the overalbest configuration varies for different video snippets for person and face detection AU for HMDB dataset, while \figref{fig:olympics} shows the same for the Olympics dataset. Since, best-tuning configurations scatter throughout the space with very little overlap, each video-snippet emulating a particular environment and camera-setting requires different tuning to achieve best analytical quality.

%entire video  for a video-snippet must provide overall best analytic quality across all frames in the video-snippet. We use detection AU (e.g., face and person detection AU) on 19 video snippets from HMDB dataset~\cite{Kuehne11} and 11 video snippets from Olympics dataset~\cite{niebles2010modeling} after manually annotating face and person bounding boxes using the cvat-tool~\cite{cvat}~\footnote{both datasets were originally used for action-recognition but due to unavailability of video-dataset for face and person detection, we use these two datasets.} 

%\figref{fig:hmdb51} shows how the overall best configuration varies for different video snippets for person and face detection AU for HMDB dataset, while \figref{fig:olympics} shows the same for the Olympics dataset. Since, best-tuning configurations scatter throughout the space with very little overlap, each video-snippet emulating a particular environment and camera-setting requires different tuning to achieve best analytical quality.

\tabref{tab:best-video-conf} shows the maximum and average analytical quality improvement achieved after tuning each video-snippet as per their best virtual knob configuration. We observe that up to 58\% improvement in accuracy of insights is possible when camera parameters are modified appropriately. 

%Each video snippet in Olympics and HMDB dataset are compressed heavily. The person detection AU, which is more coarse-grained (it looks at a much larger area with more pixels in the frame to detect a person) can tolerate such lossy compression better than fine-grained, face detection AU. Fine-grained, face detection AU (looks for much smaller space in the frame i.e. fewer pixels to detect faces) provides less improvement in detection of faces compared to person detection AU, as shown in ~\tabref{tab:best-video-conf}.

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/hmdb51_face.pdf}
    \caption{Face Detection}
    \label{fig:hmdb_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/hmdb51_person.pdf}
    \caption{Person Detection}
    \label{fig:hmdb51_person}
\end{subfigure}
\caption{Distribution of best configurations for different AUs on \emph{HMDB} video snippets}
\label{fig:hmdb51}
 \vspace{-0.2in}
\end{figure}

%\begin{figure*}
%\def\tabularxcolumn#1{m{#1}}
% \begin{tabularx}{\linewidth}{@{}cXX@{}}
% \begin{tabular}{cc}
% \subfloat[HMDB51-FaceDetection]{\includegraphics[width=8cm]{figs/hmdb51_face.pdf}\label{fig:hmdb_face}}
% & \subfloat[HMDB51-PersonDetection]{\includegraphics[width=8cm]{figs/hmdb51_person.pdf}\label{fig:hmdb51_person}
% }
% \end{tabular}
% \end{tabularx}
% \caption{Camera Best Configuration variation for different AU on \emph{HMDB51} video snippets}
%  \label{fig:hmdb51}
% \end{figure*}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/olympics_face.pdf}
    \caption{Face Detection}
    \label{fig:olympics_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/olympics_person.pdf}
    \caption{Person Detection}
    \label{fig:olympics_person}
\end{subfigure}
\caption{Distribution of best configurations for different AUs on \emph{Olympics} video snippets}
\label{fig:olympics}
 \vspace{-0.2in}
\end{figure}
 
% \begin{figure*}
%\def\tabularxcolumn#1{m{#1}}
% \begin{tabularx}{\linewidth}{@{}cXX@{}}
% \begin{tabular}{cc}
% \subfloat[Olympics-FaceDetection]{\includegraphics[width=8cm]{figs/olympics_face.pdf}\label{fig:hmdb_face}}
% & \subfloat[Olympics-PersonDetection]{\includegraphics[width=8cm]{figs/olympics_person.pdf}\label{fig:hmdb51_person}
% }
% \end{tabular}
% \end{tabularx}
% \caption{Camera Best Configuration variation for different AU on \emph{Olympics} video snippets}
%  \label{fig:olympics}
% \end{figure*}
 
\begin{table}[h!]
\begin{tabular}{||c|c||c|c|c|}
    \hline
    Video-Dataset & AU & \multicolumn{2}{c|}{mAP}\\
    & & \multicolumn{2}{c|}{improvement}\\
    \cline{3-4}
    & & Max & Mean \\
    \hline
    \multirow{2}{*}{Olympics} & Face Detection  & 19.23 & 1.68  \\
    \cline{2-4}
    & Person Detection & 40.38 & 8.38 \\
    \hline
    \multirow{2}{*}{HMDB} & Face Detection  & 18.75 & 4.22  \\
    \cline{2-4}
    & Person Detection & 57.59 & 12.63 \\
    \hline
\end{tabular}
\caption{Best configuration Accuracy Improvement}
\label{tab:best-video-conf}
 \vspace{-0.3in}
\end{table}

The camera parameter settings that provide the best improvement in accuracy of insights from analytics units are impossible for a human to identify because the best combination will vary with location of the camera, the type of analytics units, and the environmental conditions. Humans cannot keep adjusting these parameters manually, and methods to automatically and dynamically tune camera parameters are required to improve the accuracy of insights from analytics units. We describe such a system in the next section.

==> oldfiles/background.tex <==
\section{background}

\subsection{Video-Camera Pipeline}
\label{sec:video-camera-pipeline}
\figref{fig:pipeline} shows the processing pipeline within a camera. First, photons from the external world reach the image sensor, which uses a bayer filter~\cite{bayer1976color} to create the raw-image data. Then, this raw-image data undergoes various post-processing e.g. demosaicing, denoising, white-balance, color-correction, sharpening, change in brightness, contrast, color-saturation or hue, high-dynamic range and compression (i.e., JPEG/PNG or video compressions like H.264~\cite{x264}, VP9~\cite{vp9}, MJPEG, etc.) in image-signal processing (ISP) stage~\cite{ramanath2005color} and then results in human-readable encoded format. These post-processed and compressed images or video-frames are then pushed through AUs (e.g. detectors, classifiers, recognizers, etc.) to obtain desired analytical information.

%These post-processed and compressed images or video-frames are then pushed to either any detector or classifier employing convolution neural network on those input frames to obtain desired analytical information.

There are numerous parameters at different stages that affect the quality of produced image. For example, at image-sensor stage, parameters to change the amount of light that hits the sensor, to change the zoom level or field-of-view, while at ISP stage, parameters to change the color-saturation, brightness, contrast, sharpness, gamma, acutance, etc.

%There are numerous parameters either in image-sensor stage while capturing the raw-image data which change the amount of light hit the sensor, zoom and field-of-view or in ISP stage through changing color-saturation, brightness, contrast, sharpness, gamma and acutance.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/processing-pipeline.png}
    %\vspace{-0.2in}
    %\caption{Processing pipeline in camera}
    \caption{$\approach$ Overview}
    \label{fig:pipeline}
    %\vspace{-0.3in}
\end{figure}
%\vspace{-0.2in}

\subsection{Camera Parameters}
\label{sec:cam-tuning-params}
\figref{fig:pipeline} shows the processing pipeline within a camera. 
Photons from the external world reach the image sensor through an optical lens. The image sensor  uses a bayer filter~\cite{bayer1976color} to create the raw-image data, which is further enhanced by a variety of image processing techniques~\cite{ramanath2005color} like  demosaicing, denoising, white-balance, color-correction, sharpening and image compression (JPEG/PNG or video compression using H.264~\cite{x264}, VP9~\cite{vp9}, MJPEG, etc.) before a frame is retrieved from the camera. The camera manufacturer exposes many parameters  that can be set to control the image generation process. To illustrate the proposed dynamic tuning approach,  we consider four popular parameters that are common to almost all cameras. Please note that other camera parameters can also be dynamically tuned using the $\approach$ system.  The four camera parameters we consider in this paper are as follows:
%change the pixel intensity as well as \textit{image-appearance}, are as follows:

\if 0
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/phy-camera-pic.PNG}
    %\vspace{-0.2in}
    \caption{Physical Camera Knobs}
    \label{fig:phy-knobs}
    %\vspace{-0.1in}
\end{figure}
\fi

 \begin{enumerate}
 \item \textbf{Brightness:} This parameter allows us to augment images ranging from complete dark to white-washed.
 \if 0
 Brightness of an image(/frame) can be changed applying the following transformation
 \begin{align*}
     O & = clamp[(1 -\alpha)D + \alpha\ I] \\
       & = clamp(\alpha\ I); \alpha \in [0,1]\\
     \text{where O} & = \text{transformed output; I = original Image} \\
     \text{D} & = \text{Dark Image; }\alpha\ \text{= brightness factor}
 \end{align*}
 $\alpha < 1$ produces a darker image, with $\alpha > 1$, it generates a brighter image.
 \fi

 \item \textbf{Contrast:} It provides the difference between the maximum and minimum pixel values in an image. It also indicates distinguishability of a particular object within the image. 
 \if 0
 Contrast of an image can be changed by a factor $\alpha$ as follows:
 \begin{align*}
     m & = \frac{1}{h.w} \sum_{i}^{h}\sum_{j}^{w} I_{ij} \\
     D & = \text{Image filled with m} \\
     O & = clamp[(1 -\alpha)D + \alpha\ I]
 \end{align*}
 $\alpha = 0$ produces a gray image, with $\alpha < 1$, it generates an image with less contrast.
 \fi
 \item \textbf{Color-Saturation:} Saturation or Hue indicates \emph{purity} of a color inside an image. Reduced saturation contains more gray with less pure colors. 
 \if 0
 Applying following transformation, color-Saturation of an image can be changed by a factor $\alpha$ 
 
\begin{align*}
    O & = clamp[(1 -\alpha)D + \alpha\ I]; D = I_{gray} \\
I_{gray} & = I(r) + I(g) + I(b) \\
     \text{where $I_{gray}$} & = \text{grayscale version of I } \\
    \text{I(r), I(g), I(b)} & \text{ are R, G, and B pixel intensities respectively}
\end{align*}
\fi


 \item \textbf{Sharpness:} Sharpening an image enhances the edges around every object inside that image.
\if 0
\begin{align*}
K = \frac{1}{13}
\begin{bmatrix}
1 & 1 & 1\\
1 & 5 & 1\\
1 & 1 & 1 \\
\end{bmatrix}
\end{align*}
\begin{align*}
D & = I \otimes K \\
O & = clamp[(1 -\alpha)D + \alpha\ I] \\
\text{where D } & = \text{smoothed version of original image}
\end{align*}
%With $\alpha < 1$, it generates a blurred image, while $\alpha > 1$ produces image with sharpened object edges.
\fi
\end{enumerate}
Although $\approach$ focuses on these four camera parameters, $\approach$'s methodology can used to dynamically and automatically tune other complex sensors' parameters. 




==> oldfiles/conclusion.tex <==
\section{Conclusion}
Complex sensors like video cameras have tens of configurable parameters that can be set by end-users to customize the sensors to specific application scenarios. These parameter settings have a significant impact on the quality of the sensor output, and the accuracy of insights derived from sensor data. However, most end-users use a fixed parameter setting because they lack the skill or understanding to appropriately configure these parameters. We proposed $\approach$, which is a system to automatically, and dynamically adapt the complex sensor to changing environmental conditions. Such dynamic tuning is done while the application has been deployed and is in service in the real world. We show that by automatically, and dynamically updating the parameter settings to adjust to changing environmental conditions near the sensor, our system can significantly improve the accuracy of inferred insights. Also, our proposed sensor modelling and dynamic tuning methodology can be used to automatically, and dynamically tune other complex sensors. 


%Real-time video analytics applications at edge are increasing due to recent advancements in computer vision, deep learning, edge computing, 5G, etc. Video feed captured by city-wide, ubiquitous edge-cameras, however, experience different environment not only throughout the day, but also across different seasons and over various deployment areas. This variations in environment during frame-acquisition, deteriorates the performance of video analytics tasks significantly. In this paper, to combat this performance degradation, we proposed $\approach$, which continuously tunes camera parameters, using Reinforcement Learning (RL) techniques, and adapts to changing environmental conditions. As part of designing $\approach$, in order to study the problem, devise RL algorithm and rapidly test it before actual deployment, we propose a new \emph{virtual camera simulator} that not only simulates different environment conditions without changing scene-content, but also provides flexibility to try different parameter settings and different reward functions on same scene. 
%To find out the digital range of those four physical camera parameters, we define \emph{digital-twin} for each parameter.  
%We evaluate the performance of $\approach$ on two different video analytics tasks and show that it provides 11 \% accuracy improvement without impacting latency of analytical pipeline. 

%In this paper, we devise a methodology that automatically and dynamically adapt camera parameter settings to continuous environment changes. Although $\approach$ focuses on four image-appearance based parameters for RGB camera sensors but this $\approach$ can easily be extensible and generalizable for different sets of image and video-specific tunable parameters exposed by different types of camera sensors. 

%In this work, weintroduced AQuA to judge frames and assign an analytical qual-ity score. We also proposed that AQuA can be used as a filter todrop low quality fr

==> oldfiles/design.tex <==
\section{System design of $\approach$}
%Discuss high level design first and then provide details, including details of our RL based approach.

\begin{figure}[b]
 \centering
    \includegraphics[width=0.99\linewidth]{figs/system-design.png}
    \caption{$\approach$ System design}
    \label{fig:system_design}
\end{figure}

%\begin{figure*}
%\centering
%    \includegraphics[width=\textwidth]{figs/system_design.PNG}
    %\vspace{-0.2in}
%    \caption{Basic Control Loop to modify Camera Parameters}
%    \label{fig:system_design}
     %\vspace{-0.1in}
%\end{figure*}
 
 \figref{fig:system_design} describes the system-level architecture for automatic, and dynamic tuning of camera parameters. Live video streams from the camera are processed at the edge by a lightweight AQuA module~\cite{paul2021aqua} to discard low-quality frames. These frames are not suitable for analytics, and early discard helps to reduce the required wireless network bandwidth. At the edge of the wireless network, the video stream is mined for insights by using analytic units. An AU-specific analytics quality estimator detects a change in analytics quality, if any, and communicates with a reinforcement learning module that dynamically, and remotely, adjusts the camera parameter settings. 
 %These frames do not contribute to AU accuracy improvement or camera-parameter tuning 
%$\approach$'s system design, including control loop to modify and tune camera parameters in a network camera in order to improve the AQ for a given AU is shown in \figref{fig:system_design}. Live-video feeds are continuously being captured by the image sensor at network camera from external environment, then various image-processing techniques are applied through ISP pipeline to obtain the final processed frame. Before offloading it to edge-server or remote-cloud for further analytics using wireless network (i.e. 4G or 5G), these processed frames are filtered by lightweight \emph{AQuA-filter}~\cite{paul2021aqua}, which discards low-quality frames, which might might lead to high-confidence errors (i.e. not suitable for AU). This also helps to reduce wireless network bandwidth requirement through early-discard of frames that do not contribute to AU accuracy improvement or camera-parameter tuning for better analytics.

%On the edge server, filtered and offloaded frames are parallelly passed through different analytic pipeline and fine-grained AU-specific analytics quality estimator. We can simply employ the analytic analytics quality estimators described in ~\secref{sec:motivation} specific to each AU i.e., \textit{joint mAP and IoU metric} for any detection AU, \textit{match-score} for face-recognition AU, \textit{RMS distance} between predicted and actual keypoints in case of keypoint detection. But all these estimators require ground-truths (or labeled data), that is not possible during runtime unless we keep a human in the control loop that continuously labels the incoming frames for several analytics, which is not practical.

Detecting a change in accuracy of insights from the analytics unit is a difficult task. Since no ground truth is available during normal operation of the streaming system, we design a proxy that estimates the accuracy of insights. Design of the AU-specific analytics quality estimator is described in Section~\ref{sec:AU-specific}. A reinforcement learning module reacts to a change in analytical quality estimates, and dynamically adjusts the camera parameters to improve the accuracy of insights. Section~\ref{camera-parameters-tuning} describes the reinforcement learning module.

%As a substitute to generating the ground-truth (not possible in an actual deployment), which can be used for determining the AU quality, we introduce a fine-grained proxy analytics quality estimator. This proxy quality estimator is AU-specific and provides a quality estimate that can be used to determine the quality of offloaded frame. Based on the AU quality, determined from the proxy analytics quality estimator, the camera parameters are tuned automatically, so as to improve the AU quality further. Camera vendors provide APIs e.g. \emph{Axis provides VAPIX}~\cite{vapix}, through which we can change the camera parameters programmatically. It typically takes a very short time (around 150 to 200 milliseconds) to change the parameters, so this approach is feasible in dynamically tuning camera parameters. This tuning process continues over the lifetime of the AU. Specifically, we use Reinforcement Learning (RL) technique to tune the camera parameters. RL requires a reward function, using which it continuously decides which next actions to take. ~\secref{sec:AU-specific} discusses how to train AU-specific custom analytics quality estimator model that can provide continuous reward function (without any ground-truth labelling during runtime) to RL, which we discuss in section \ref{camera-parameters-tuning}
%discuss what we are going to tell in 5.1 and 5.2

%To reduce human-effort in tuning the camera knobs and make it automatically tunable, we here introduce a fine-grained proxy analytics quality estimator. This AU-specific analytics quality estimator provides a quality estimate that acts as a reward value for the reinforcement learning (RL)~\cite{}. State for RL includes current and previous values of brightness, contrast, sharpness and color-saturation. Depending on the measured state and reward value, RL algorithm can take one of 9 actions those include increase or decrease each of the four tuning knobs independently or no change at all.

%\textcolor{red}{please add further details of the reinforcement learning}
%\textcolor{blue}{we can bring in SARSA description and define what our state, action and rewards are ..}

\subsection{AU-specific analytics quality estimator}
\label{sec:AU-specific}
%correlation between actual ground-truth metric and quality metric
As described in Section~\ref{sec:knob-impact}, methods to estimate the accuracy of insights from analytics units depend on the function of the analytics unit. For example, a combination of mAP and true-positive IoU is typically used to estimate the accuracy of insights from a face or person detection AU, while true-positive match-score is the preferred analytical quality metric for a face recognition AU. Similarly, a common analytical quality metric for key-point detection AU is the root-mean-square distance between the predicted and actual landmarks. All these analytical quality metrics assume availability of ground-truth, which  is compared with the predicted outputs from the analytics units. 

Since no ground truth is available in a real-world deployment, we need a different approach to estimate analytical quality. We propose training a deep-learning model to predict analytical quality estimates for an analytics unit. We trained two different AU-specific analytical quality estimators, and we briefly describe these models.  

%Our first inclination was to use AQuA~\cite{paul2021aqua} scores as a proxy for the analytical quality estimates. 
%To use existing AQuA-filter~\cite{paul2021aqua} as a proxy quality estimator for RL agent, we first examine the correlation between AQuA predicted quality and different analytical quality (AQ, described in ~\secref{sec:knob-impact}). The weak correlation (i.e., spearman correlation $\approx$ -0.03) between AQuA predicted quality and AQ propels us to design \emph{AU-specific Analytics Quality Estimator} that provides a fine-grained continuous quality measure (i.e., reward function for RL algorithm) for any offloaded frame filtered by AQuA. These quality-estimator models are defined and trained for three different AUs, as follows:

\begin{itemize}
    \item \textbf{Estimator for Face-recognition AU :} For 300 randomly-sampled celebrities from celebA dataset~\cite{liu2015faceattributes}, we choose two images per person. We use one of them as a reference image and add it to the gallery. We use the other image to generate multiple variants by changing the virtual knob-values. These variants are the query images ($\approx$ 4M query images). For each query image, we obtain the match score (which is a value between 0 and 1) by using the Face recognition AU. The query images along with their match score are the labeled examples we use to train a deep-learning model, which will predict the match score for an image. We trained a deep-learning model (network architecture is similar to the lightweight AQuA network) with 101 output classes. One of the classes signifies no match, while the remaining 100 classes correspond to a match score between 1 to 100. 
    %constitutes training dataset for the analytics quality estimator model. Each of these query images when sent to the face-recognition model, provides a celebrity name with a matchScore between [0,1]. For every correct face-recognition, we use the corresponding rounded value of \underline{\emph{matchScore*100}} as the class-label. Total 101 classes can be there in the training dataset. Hence, we train the existing AQuA model with 101 output nodes.
    
    \item \textbf{Estimator for person \& face detection AU :} We used Olympics~\cite{niebles2010modeling} and HMDB~\cite{Kuehne11} datasets, and created $\approx$ 7.5M variants of the video frames. Then, we used the AUs to determine the analytical quality estimate, which is a combination of mAP and IoU values (as shown in Equation~\ref{eq:detection}). The video frames, and their quality estimates, are the labeled examples, and we trained a deep-learning model (again, the network architecture is lightweight and similar to AQuA network) with 201 classes to predict the analytical quality estimate for a video frame. 
    
    
   % To design analytics quality estimator specific to these detector AUs, we train AQuA classifier model with 201 output nodes on the Olympics~\cite{niebles2010modeling} and HMDB~\cite{Kuehne11} training video frames and their augmented variants ($\approx$ 7.5M). While training, each frame is associated with a classlabel based on the joint-metric of mAP and the IoU for true-positive detections as shown in equation~\ref{eq:detection}. Hence, higher the classlabel, better is the analytic quality. 
    \begin{equation}
    \label{eq:detection}
    classlabel \leftarrow mAP + IOU_{True-Positive}*100
    \end{equation}
    \end{itemize}



    \if 0
    \item \textbf{Facial-Keypoint Detection AU :} Out of 300 outdoor images in 300W dataset~\cite{}, 200 randomly selected images and their augmented variants are used as the training dataset ($\approx$ 2M). Each of these images are passed through the facial-keypoint detector. We then discretize the RMS distance obtained between the predicted and ground-truth keypoints into 500 different classes. Class-label is determined using equation~\ref{eq:facial-kp}. Similarly, we train the existing AQuA model with 500 output nodes to obtain \emph{facial-keypoint detection AU-specific AQuA classifier model}.

\begin{equation}
\label{eq:facial-kp}
classlabel \leftarrow 499 - Max(round(dist_{RMS}(predicted,gt)*5), 499)
\end{equation}    
\fi

\subsection{Reinforcement Learning}
\label{camera-parameters-tuning}
To automatically tune the camera parameters, we use reinforcement learning (RL) \cite{introduction-to-rl} techniques. We use State-Action-Reward-State-Action (SARSA) RL algorithm~\cite{q-lambda}. In this setup, there is an agent, which interacts with the environment (\textit{state}) it is in, by taking different \textit{actions}. As the agent takes actions, it moves into a new state or environment. For each action, there is an associated \textit{reward} or penalty, depending on whether the new state is desirable or not Over a period of time, as the agent continues taking actions and receiving rewards and penalties, the agent learns to maximize the rewards by taking the right actions, which ultimately leads the agent towards desirable states.

SARSA does not require any labeled data or pre-trained model, rather it learns and updates its policy based on the action it takes. Therefore, it is an on-policy learning algorithm and requires a clear definition of the environment (state), actions and reward. For the purpose of automatic camera-parameter tuning, we define them as follows:

%\textit{State}: This is a vector containing the following quantities:
%\begin{itemize}
%    \item Current brightness parameter value on the camera
%    \item Current contrast parameter value on the camera
%    \item Current sharpness parameter value on the camera
%    \item Current color parameter value on the camera
%    \item Measure of brightness
%    \item Measure of contrast
%    \item Measure of sharpness
%    \item Measure of color
%\end{itemize}

\textit{\underline{State}}: This is a vector containing (a) the current brightness, contrast, sharpness and color parameter values on the camera and (b) measure of brightness, contrast, sharpness and color-saturation.

%\textit{Action}: The set of actions that the agent can take are:
%\begin{itemize}
%    \item Increase brightness parameter value
%    \item Decrease brightness parameter value
%    \item Increase contrast parameter value
%    \item Decrease contrast parameter value
%    \item Increase sharpness parameter value
%    \item Decrease sharpness parameter value
%    \item Increase color parameter value
%    \item Decrease color parameter value
%    \item Don't take any action
%\end{itemize}

\textit{\underline{Action}}: The set of actions that the agent can take are (a) increase or decrease one of the brightness, contrast, sharpness or color-saturation parameter value or (b) not take any action at all.

\textit{\underline{Reward}}: We use the AU-specific analytics quality estimators as the reward function for SARSA algorithm. If the quality estimate improves, then it is considered as a reward, whereas if the estimate decreases, then it is considered as a penalty.

The reward obtained by using the proxy analytics quality estimator is termed as the immediate reward. Along with considering immediate reward, the agent also factors in future reward that may accrue as a result of the current actions. Based on this, a value, termed as Q-value is calculated for taking an action $a$ when in state $s$. This is denoted as $Q(s,a)$. The value for $Q(s,a)$ is calculated as per Equation \ref{eq:sarsa}. Here, $\alpha$ is a constant with a value between 0 and 1. This can be used to control how much importance is to be given to new information obtained by the agent. A value of 1 will give high importance to the new information while a value of 0 will stop the learning phase for the agent. During the initial phase, a higher value e.g. 0.9 can be assigned by the operator, which will help the agent quickly \textit{learn} and understand the new environment by giving higher importance to the most recent information. After the agent has learnt and assimilated the information from the new environment, the value of $\alpha$ can be lowered e.g. 0.1 by the operator so that the agent now starts \textit{using} the gathered information about the new environment. 

\begin{equation}
\label{eq:sarsa}
Q(s,a) \leftarrow Q(s,a) +
\alpha \left[ r + \gamma \cdot Q(s^\prime, a^\prime) - Q(s,a) \right]
\end{equation}

Similar to $\alpha$, there is another constant $\gamma$ in equation \ref{eq:sarsa}, which has a value between 0 and 1. This constant is called as the discount factor and can be used to control the importance given by the agent to any long term rewards. A value of 1 will give very high importance to long term rewards while a value of 0 will make the agent ignore any long term rewards and focus only on the immediate rewards. If the conditions change very frequently then a lower value e.g. 0.1 can be assigned to $\gamma$ so as to prioritize immediate rewards, while if the conditions do not change frequently, then a higher value e.g. 0.9 can be assigned to prioritize long term rewards.

The steps followed by an agent are shown in Algorithm \ref{alg:sarsa}. Here, the agent first observes the environment i.e. state $s$ and chooses an appropriate action $a$ to be performed in state $s$. After performing the action $a$, the agent receives an immediate reward (or penalty) $r$ and is now in a new state $s'$. In this new state, the action chosen by the agent is $a'$ and the associated Q-value is $Q(s',a')$, which the agent uses to compute the cumulative reward $Q(s,a)$ as per equation \ref{eq:sarsa}. The agent then updates this computed cumulative Q-value and is now in the new state $s'$. This process continues for the lifetime of the AU as the agent continuously learns and adapts to the environment.

\begin{algorithm}[t]
\DontPrintSemicolon
\SetKwFunction{OE}{Observe-Environment}
\SetKwFunction{CA}{Choose-Action}
\SetKwFunction{SP}{Still-Processing}
\SetKwFunction{PA}{Perform-Action}
\SetKwFunction{CR}{Compute-Reward}
\SetKwData{S}{s}
\SetKwData{SPRIME}{s'}
\SetKwData{A}{a}
\SetKwData{APRIME}{a'}
\SetKwData{Q}{Q}
\SetKwData{R}{r}
\SetKwData{ALPHA}{alpha}
\SetKwData{GAMMA}{gamma}

\S $\leftarrow$ \OE{} \;
\A $\leftarrow$ \CA{\Q, \S} \;
\While{\SP{}}{
    \PA{\A}\;
    \R $\leftarrow$ \CR{} \;
    \SPRIME $\leftarrow$ \OE{}\;
    \APRIME $\leftarrow$ \CA{\Q, \SPRIME} \;
    \Q(\S, \A) $\leftarrow$ \Q(\S,\A) + \ALPHA $\times$ [\R + \GAMMA $\times$ \Q(\SPRIME, \APRIME) – \Q(\S, \A)] \;
    \S $\leftarrow$ \SPRIME \;
    \A $\leftarrow$ \APRIME \;
}
\caption{State-Action-Reward-State-Action loop}
\label{alg:sarsa}
\end{algorithm}

\begin{algorithm}[t]
\DontPrintSemicolon
\SetKwFunction{RND}{rand}
\SetKwFunction{RA}{Random-Action}
\SetKwFunction{REV}{Revert}
\SetKwFunction{MA}{Max-Action}
\SetKwFunction{CR}{Compute-Reward}
\SetKwData{S}{s}
\SetKwData{SPRIME}{s'}
\SetKwData{A}{a}
\SetKwData{APRIME}{a'}
\SetKwData{Q}{Q}
\SetKwData{R}{r}
\SetKwData{ALPHA}{alpha}
\SetKwData{EPS}{epsilon}
\SetKwInOut{Input}{Input}

\Input{\Q,\S,\A,\R}
\If{\RND{0,1} $\geq$ \EPS} {
    \Return \RA{}
}
\If{\R $<$ 0} {
    \Return \REV{\A}
}
\APRIME $\leftarrow$ \MA{\Q, \S} \;
\If {\R $>$ \Q(\S,\APRIME)} {
    \Return \A
}
\Return \APRIME
\caption{Policy for choosing the action to perform}
\label{alg:policy}
\end{algorithm}

While algorithm \ref{alg:sarsa} provides the steps followed by the agent, it does not provide the exact method used by the agent to choose the action $a$ to be performed. For this, we devise a \emph{new} policy for the agent to decide the action to be performed. This policy is shown in algorithm \ref{alg:policy}. We define a constant called \textit{epsilon} which has a value between 0 and 1 and can be tweaked by the operator. Initially, the agent generates a random number between 0 and 1. If the random number is greater than the set value of \textit{epsilon}, then a random action is chosen. As we can see, lower value of \textit{epsilon} will trigger more random actions to be generated while higher value of \textit{epsilon} will trigger less random actions. Therefore, during the initial phase of the deployment, when the agent explores various actions, typically the value of \textit{epsilon} is set lower e.g. 0.1, while after the agent has explored enough, the value of \textit{epsilon} is set higher e.g. 0.9, so that the agent starts using the learned information from the earlier exploration phase and starts exploiting it. If the random number is lower than the set value of \textit{epsilon} then the reward $r$ is checked. If the reward is less than 0 i.e. if the action results in a penalty, then the action is reverted immediately. However, if the reward is positive but less than the predicted reward for the action, then the same action is repeated. Thus, this is a greedy policy where the actions leading in positive direction are repeated while the action leading in negative direction are immediately reverted.

%Under continuous inferior-quality frame acquisition due to camera-misconfigurations, AQuA-filter passes one intermediate frame to AU-agnostic analytics quality evaluator after every \emph{K} continuous inferior-quality frames. This enables RL agent to tune camera parameter adapting to environmental condition.

It may happen sometimes that due to extremely poor capture from the camera (due to sudden change in environment e.g. lights being turned off in an indoor setting), most of the frames get dropped by AQuA-filter. In such cases, without any frames being sent to $\approach$, RL agent will not be able to take any corrective actions. To avoid this scenario, we designed AQuA-filter in such a way, that after every configurable number of successive frames being dropped, 1 frame is sent to AU-specific Analytics Quality Estimator, so that $\approach$ is aware of actual frames being produced by the camera and can take appropriate action.  


% Under continuous inferior-quality frame (i.e., provide high-confidence erroneous predictions by AU) capture and early-discard due to camera-misconfiguration, AQuA-filter passes one intermediate frame after K continuous inferior-quality frames. This enables RL agent to take required action in order to 












==> oldfiles/evaluation.tex <==
\section{Evaluation}
%Provide detailed evaluation methodology, various experiments that were performed, results without using our RL approach and then results with our RL approach. Show that our RL approach helps in improving AU accuracy.
%we can then provide the timing analysis, how each block impacts the timing.
We discuss our evaluation methodology and describe our performance evaluation results for the three main components:  virtual camera, AU-specific analytics quality estimator and SARSA RL agent. We then analyze the overall system performance through a real-world deployment.

\subsection{Evaluation methodology}
\label{sec:eval-method}
We loop a pre-recorded (original) video through two virtual cameras. For the first virtual camera, we gradually change the model parameters to simulate the changes that happen during the day as the sun changes its direction and finally sets. This way, the video feed coming out from the first virtual camera mimics the conditions that would have occurred as the lighting changes from daylight to evening, to twilight, to dusk and finally night. Under this gradual change in light conditions, we continuously measure the accuracy of the insights from the AU. The first virtual camera is not controlled by the RL module, and results from the first virtual camera video feed are our baseline. For the second camera, we also gradually change the model parameters to simulate the lighting changes that would have occurred during the day, but on this second virtual camera, we also adjust the virtual knobs  dynamically by using our reinforcement learning module. Then, we compare the accuracy of insights from the AU to the baseline results. 
%where in one scenario we do not apply our technique, while in the other scenario, we apply our technique and tune camera parameters dynamically.

Note that in our experiment, it is important to choose a good quality video as original video.
%which was captured at broad daylight, because it is possible to recover and restore from good quality video when we apply our technique.
If we start with a poor quality video (for example, night video with poor lighting), then the output video from the virtual camera does not have enough information; so no matter how much we adjust the virtual knobs, it wouldn't help. This jives with the fact that in actual deployment, our technique would constantly monitor the conditions and keep tuning camera parameters (from daylight all the way to night) so that the camera feed is of reasonably good quality at all times. By using our technique, we avoid the situation where the video feed coming out of the real camera is of exceptionally poor quality.

\subsection{Training}
We train AU-agnostic AQuA-filter by using the lightweight inception-v3~\cite{szegedy2016rethinking} backbone until the first inception block~\footnote{AQuA-filter uses only 14\% of total model-size of Inception-v3} by using the validation images from ImageNet ILSVRC-2017 dataset~\cite{deng2009imagenet} and their augmented variants. Along with 7 different distortions mentioned in ~\cite{paul2021aqua}, we also train AQuA for color-saturation and sharpness variations. 

AU-specific analytics quality estimators use a similar network as AQuA. However, these estimators have different number of output nodes (or classes) for different AUs. 
%It classifies the offloaded filtered frame into one class as opposed to AQuA-filter (with one output node) which regresses to one quality value for any input frame.
We use cross-entropy loss function to train AU-specific estimators, while the AU-agnostic AQuA model is trained using MSE loss.
All models are trained end-to-end with an initial learning rate of $10^{-5}$ and we use the Adam Optimizer~\cite{kingma2014adam}.
%We use transfer learning to train both AQuA classifier and regressor. 
%The mobilenetv2 (i.e., AQuA-filter) or inception-v3 (until 1 inception block)-based feature extractors are initialized using weights from an ImageNet trained respective models (mobilenetv2 or Inception-v3 model), and are frozen. While training, only the weights in the fully connected regression layers for AU-agnostic AQuA or classification layers for AU-specific AQuA are updated.
%The model is trained end-to-end with an initial learning rate of $10^{-5}$ and using the Adam Optimizer~\cite{kingma2014adam}. 

%For training the model to automatically tune camera parameters using Reinforcement Learning, as described in section \ref{camera-parameters-tuning}, we use SARSA algorithm, in which the agent learns to maximize the reward, thereby creating a model which adjusts and adapts to the changing environmental conditions. \textcolor{black}{Use of VC simulator and virtual knobs make training of this RL module significantly faster (greater than 10x speedup)}.
%\textcolor{red}{Mention training of RL model}


\subsection{Virtual camera}
%We first evaluate how well VC re-renders scenes from a good quality input video to mimic different environmental conditions. We take a 5-minute long video (taken at an hour, $H_1$) and convert the video capture time (i.e., output time) into 23 other hours (excluding the original video capture hour) by applying VC simulator (also shown in algorithm~\ref{alg:vc-sim}). We then extract the four image-features <brightness, contrast, colorfulness, sharpness> of the transformed video frames and compare with the extracted image-features obtained of the frames captured during the transformed output hour. We repeat this validation process for few other videos (taken at an hour different from $H_1$). ~\tabref{tab:eval-vc} shows the mean error and its standard deviation between the transformed frame features and original frame features (i.e., captured at the modified output time). While transformed frames' brightness closely replicate the brightness of original frames with an error of 5.4\%, an error around 20\% is observed for sharpness image feature. With the help of this close-approximation of VC simulator while transforming the frames, we can able to evaluate the performance of our RL agent on various external-environment conditions experienced by any network camera throughout the day.

VC should faithfully render a frame from time $T1$ to any other time $T2$, as if it was actually captured at time $T2$. In order to evaluate if VC is able to do this, we obtain several video snippets at different hours of the day. Then, we run these video snippets through VC and generate 23 other video snippets (for other hours of the day). We then compare the values of feature tuple of the generated video snippets through VC (transformed) and the values of feature tuple from the video snippets actually captured at those hours (original). ~\tabref{tab:eval-vc} shows error and standard deviation between the transformed and original videos. We note that average VC error is under 20 \% for brightness, contrast, color-saturation and sharpness.

\begin{table}[h!]
 \centering
 \begin{tabular}{|c|c|c|c|c|}
 \hline
Brightness & Contrast & Color & Sharpness \\
& & -Saturation & \\ \hline
\SI{5.4 \pm 1.7}{\percent} & \SI{13.8 \pm 4.3}{\percent} & \SI{17.3 \pm 9.6}{\percent} & \SI{19.8 \pm 8.1}{\percent} \\
\hline 
 \end{tabular}
 \caption{VC error}
 \label{tab:eval-vc}
 \vspace{-0.3in}
 \end{table}



\subsection{AU-specific analytics quality estimator}
%In absence of ground-truth labelling during runtime, \approach\'s RL agent takes any action based on the continuous quality value measured on offloaded frame by AU-specific analytics quality (i.e., AQ) Estimator (also shown in ~\figref{fig:system_design}). 
We evaluate the performance of AU-specific estimators by determining the correlation between predicted quality estimates and the analytical quality estimates derived using ground-truth. ~\figref{fig:au_corr} shows the Spearman and Pearson correlation metric for three different AUs. The match-score for celebA-validation images with its augmented variants ($\approx$2M) and predicted quality by face-recognition-specific analytics quality estimator is strongly correlated (Pearson and spearman correlation both are greater than 0.6)~\footnote{Pearson correlation greater than 0.5~\cite{corr} and spearman correlation~\cite{corr_1} value greater than 0.6 imply strong correlation.}.
For face-detection and person-detection quality estimators, we used annotated video frames from \textit{olympics}~\cite{niebles2010modeling} and \textit{HMDB} dataset~\cite{Kuehne11} and their various variants that were generated by changing the virtual knobs. ~\figref{fig:au_corr} shows the strong positive correlation between the measured mAP and IoU metric, and the predicted quality estimate for both face-detection and person-detection AUs. This strong correlation enables $\approach$'s RL agent to tune camera parameters based on the reward value provided by AU-specific analytics quality estimator. 

\if 0
 \begin{table}[h!]
 \centering
 \begin{tabular}{|c|c|c|}
 \hline
 AU & Pearson & Spearman \\
  & Correlation & Correlation \\ \hline
 Face Recognition & 0.614 & 0.608\\ \hline
 Face Detection & 0.738 & 0.675 \\ \hline
 Person Detection & 0.574 & 0.588 \\ \hline 
 \end{tabular}
 \caption{AU-specific AQ Estimator Performance}
 \label{tab:eval-au-specific}
  \vspace{-0.3in}
 \end{table}
 \fi
 
 \begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/au_specific_impact.pdf}
    \caption{AU-specific analytics quality estimator Performance}
    \label{fig:au_corr}
     \vspace{-0.2in}
\end{figure}



\subsection{SARSA RL}
%How long RL takes to converage
We applied SARSA RL agent to tune four virtual knobs in the virtual camera pipeline (as shown in ~\figref{fig:eval_setup}) on 5-minute video segment (i.e., consists of 7500 frames)~\footnote{Ground-truth annotations are done on the video-segment to find out the actual detection accuracy (mAP) improvement.} for 6 randomly selected time segments  throughout the day (each time-segment is separated by at least 1 hour). RL agent adaptively adjusts the four virtual knobs 
%for face detection AU and person detection AU separately 
with the help of AU-specific reward function, as explained in~\secref{sec:AU-specific}, after every \emph{1 min} interval (this interval is configurable). ~\figref{fig:rl_cdf} shows the cumulative distribution function of mAP improvement for the six videos that correspond to six distinct time-segment of the day. Each point (x,y) in~\figref{fig:rl_cdf} shows that y\% of videos experience mAP improvement that is between 0 to x\%. Dynamically adjusting the four virtual knobs by using RL improves face-detection accuracy by \emph{8.31\%} on average (the mAP improvement can be as much as \emph{13.74\%}). Similarly, we notice a \emph{7.35\%} average mAP improvement for person-detection (the mAP improvement can be as much as \emph{8.95\%}).

%~\tabref{tab:rl-eval} shows the maximum and average mAP improvement for those two AUs. Tuning those four virtual knobs with RL improves face-detection accuracy by 8.31\% on average while slightly less 7.35\% average mAP improvement is observed for person-detection. 

\if 0
\begin{table}[h!]
\begin{tabular}{|c|c|c|}
    \hline
    AU & \multicolumn{2}{c|}{mAP}\\
    & \multicolumn{2}{c|}{improvement (\%)}\\
    \cline{2-3}
    & Max & Mean \\
    \hline
    Face Detection  & 13.74 & 8.31  \\
    \hline
    Person Detection & 8.95 & 7.35 \\
    \hline
\end{tabular}
\caption{Accuracy Improvement after RL parameter tuning}
\label{tab:rl-eval}
 \vspace{-0.3in}
\end{table}
\fi

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/rl_cdf.pdf}
    \caption{CDF of mAP improvement for different AUs}
    \label{fig:rl_cdf}
     \vspace{-0.2in}
\end{figure}


\subsection{Overall System Analysis}
%The virtual camera (VC) is same as actual RGB camera where depending on the capture time of the day, scene characteristics adapt to that time without changing the frame-content (explained in ~\secref{sec:vc-sim}). 
To ensure repeatability and reproducibility, we use the same scenes to evaluate the performance before and after applying $\approach$. We use a virtual camera and loop-through pre-recorded proprietary videos taken at different time-segments of day, as shown in ~\figref{fig:eval_setup}. The virtual camera continuously extracts frames from the input video and applies transformations to re-render it to emulate different time-segments of the day without changing the frame-content (explained in ~\secref{sec:vc-sim}). Before offloading to edge-server, frames are passed through the \emph{AQuA filter}. Both Virtual camera model and AQuA model are running on a low-end edge device with tiny footprint, \emph{Intel-NUC box} equipped with \textit{Intel i7-6770HQ 2.6 GHz CPU}. AQuA filter takes \emph{40 ms} processing time (with a CPU usage $\approx$ 80\%) per frame, and outputs a quality value. Depending on this quality value and threshold, inferior-quality frames are discarded and the rest are sent for analytics processing to the edge-server over a 5G network with an average offload latency of \emph{39.7 ms}. Temporal locality in captured video helps to offset AQuA computation overhead on edge device by applying AQuA-filter only on a few intermediate frames. AQuA-filter on edge device also helps to reduce the 5G bandwidth requirement by 15\%-20\%. 

On the edge-server, RetinaNet face detection AU, EfficientDet person detection AU and  AU-specific analytical quality estimators  are running on \textit{NVIDIA GeForce RTX 2070 GPU}. RetinaNet face detection AU takes \emph{86 ms} while person detection AU takes \emph{96 ms} to process each frame on a GPU (utilization  is $\approx$ 25\%). Computation time for AU-specific analytical quality estimators is only 14 ms on this GPU server.
%With the fine-grained quality value prediction by AU-specific AQuA, SARSA RL agent running on \textit{Intel i9-9980XE 3GHz CPU}, takes appropriate action to change the virtual camera image-appearance (i.e., part of post-processing) configurations after \emph{every 1min interval}. \textcolor{black}{}
SARSA RL agent (on an \textit{Intel i9-9980XE 3GHz CPU}) can perform each action within a few milliseconds by using virtual knobs, which otherwise would take several hundred milliseconds on a real camera. 
%On edge-server, AU specific AQuA classifier and RL agent are running on two different threads (in parallel and also lightweight), hence they do not impact either face detection or person detection AU performance. 
%timing granularity - 1 min
%AU-specific quality evalutator takes 14 ms
%AU-agnostic Pre-filtering on device ?? ms
%resource usage of AQuA filter
%How much time taken by different analytics unit
%face-detector, person-detector


\begin{figure}[b]
 \centering
    \includegraphics[width=0.99\linewidth]{figs/deployment-setup.png}
    \caption{Deployment Setup}
    \label{fig:real_deployment}
     \vspace{-0.3in}
\end{figure}

\subsection{Real-world deployment}
We position two cameras side-by-side so that both cameras view almost same scene at the same time, as shown in ~\figref{fig:real_deployment}. While captured frames from camera-1 are directly passed on to the AU, the frames from camera-2 are filtered using AQuA, and sent to the AU (face detection) for processing. AU-specific estimator predicts the analytical quality, and the SARSA RL agent adjusts the camera parameters by using the VAPIX API provided by the camera vendor. We compared the accuracy of insights derived from the video feeds from camera-1 and camera-2. 
%We kept this deployment running from afternoon to evening and also store the captured frames and detections to evaluate the \approach\'s performance. Later manually annotating the ground-truth, 
We observed an mAP improvement of \emph{12\%} for Camera 2's video stream.  




==> oldfiles/introduction.tex <==
\section{Introduction}
Due to the growing demand for automation and the impetus to make everything ``smart", 
the global smart sensor market size is expected to grow from US \$36 billion in 2020 to US \$88 billion by 2025, at a CAGR of 19 \% \cite{sensor-market}. Sensors are the eyes and ears of any automation system. Some sensors like pressure or temperature transducers are simple, but as more and more features are added, the complexity of the sensors is increasing. For example, complex sensors like video cameras, thermal cameras and lidars include an increasing array of features and tens of configurable parameters, which can be set by end users to customize the sensors to specific application scenarios \cite{10.3390/jimaging5100078} \cite{10.1109/ISCE.2007.4382143}. Although values for the configurable parameters determine the quality and information content in the sensor output, and this directly impacts the quality of insights obtained from AI and machine learning models that process the sensor data streams, most end-users do not have the skill or understanding to appropriately configure these parameters. Furthermore, the environmental conditions around the sensors can vary considerably \cite{10.1109/SSIAI.2018.8470354} during the lifetime of the sensor applications, and the values for the configurable parameters may have to be updated multiple times to ensure consistent, high quality sensor output and highly accurate insights from the sensor data. 


%These factors were already fueling the growth in overall Video Analytics market size in various sectors including surveillance, traffic monitoring, retail analytics, healthcare, banking, etc., but COVID-19 \cite{covid-19} accelerated the growth even further. According to a recent report, video analytics market is estimated to grow from \$5,186.0 million in 2020 to \$21,778.0 million by 2027, at a CAGR of 22.70 \%.  \cite{allied-market-research}. This estimate for 2027 was pre-COVID-19 and the projected estimates for 2027 is even higher because of sudden new demands for video analytics in order to support the measures being taken to combat the COVID-19 virus. Specifically, enforcing social distancing, administering government lockdowns and containment zones, temperature screening, limiting crowds and total number of people at any given point within a facility, recognizing individuals even with face masks, identifying demographics of people, enabling contactless transactions, payments, boarding, etc. have turned out to be new demands and video analytics is playing a major role in assisting the authorities in their day-to-day operations in handling these new and emerging COVID-19 specific scenarios~\cite{covid-vd, covid-vd-1, covid-vd-2}.


%various configuration parameters are being exposed in order to use these features. Sensor vendors think that by exposing parameters, it becomes easier for the user to tune and use the sensor. Although to some extent this is true, but to a large extent, having more parameters, means having more configuration options to deal with and that becomes a challenge in itself to find the best combination of parameters for a given analytics task to be performed. Moreover, the best combination of parameters varies with time, depending on various factors, and it is not practical to manually keep tuning these tens of sensor parameters simultaneously, especially, when thousands to millions of sensors are deployed across various deployment conditions, as is the case today.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/sensor-deployments.png}
    %\vspace{-0.2in}
    \caption{City-scale video analytics}
    \label{fig:intro}
    %\vspace{-0.1in}
\end{figure}

Using a video camera (which exposes tens of configurable parameters to end-users) as a representative complex sensor, we propose a system, called $\approach$, that automatically, and dynamically adapts the complex sensor to changing environmental conditions. Such dynamic tuning improves the accuracy of insights from video analytics. Due to the significant progress in machine learning and computer vision techniques for processing video streams~\cite{krizhevsky2012imagenet}, growth in Internet of Things (IoT), edge computing and high-bandwidth communication links like 5G~\cite{QUALCOMM-5G, CNET-5G},  video analytics market is estimated to grow from \$5 billion in 2020 to \$21 billion by 2027, at a CAGR of 22.70 \%~\cite{allied-market-research}. Cameras are increasingly being deployed throughout the world in city-scale applications like surveillance, transportation, and public safety  where different types of video analytics tasks are being performed on thousands of video feeds, as shown in Figure~\ref{fig:intro}. 
%In this paper, we use cameras as a representative sensor (which exposes tens of parameters) and propose a system, called $\approach$, which dynamically adapts to changing environmental conditions and identifies the best combination of parameter values to enhance insights from video analytics. Due to the significant progress in machine learning and computer vision techniques for processing video streams, artificial intelligence, deep learning and machine learning~\cite{krizhevsky2012imagenet}, and growth in Internet of Things (IoT) and edge computing, coupled with availability of 5G, thereby enabling low latency and high bandwidth communication~\cite{QUALCOMM-5G, CNET-5G}. 

$\approach$'s sensor modelling and dynamic tuning approach can also be used to automatically, and dynamically tune other complex sensors. For example, a thermal camera exposes several parameters like object emissivity, atmospheric transmission, and ambient temperature for temperature compensation. The proposed techniques can be used to dynamically tune these parameters as environmental conditions (like lighting, relative humidity, reflective surfaces and ambient temperature) change, and ensure consistent, highly accurate temperature measurements. 
%Also, for PTZ cameras, parameters like ``Pan", ``Tilt" and ``Zoom" need to be continuously adjusted based on analytics requirement, as the object of interest moves in the scene. 

%Video analytics has become very popular and widespread in the past decade due to advancements in computer vision algorithms, artificial intelligence, deep learning and machine learning~\cite{krizhevsky2012imagenet}, and growth in Internet of Things (IoT) and edge computing, coupled with availability of 5G, thereby enabling low latency and high bandwidth communication~\cite{QUALCOMM-5G, CNET-5G}. 
%These factors were already fueling the growth in overall Video Analytics market size in various sectors including surveillance, traffic monitoring, retail analytics, healthcare, banking, etc., but COVID-19 \cite{covid-19} accelerated the growth even further. According to a recent report, video analytics market is estimated to grow from \$5,186.0 million in 2020 to \$21,778.0 million by 2027, at a CAGR of 22.70 \%.  \cite{allied-market-research}. This estimate for 2027 was pre-COVID-19 and the projected estimates for 2027 is even higher because of sudden new demands for video analytics in order to support the measures being taken to combat the COVID-19 virus. Specifically, enforcing social distancing, administering government lockdowns and containment zones, temperature screening, limiting crowds and total number of people at any given point within a facility, recognizing individuals even with face masks, identifying demographics of people, enabling contactless transactions, payments, boarding, etc. have turned out to be new demands and video analytics is playing a major role in assisting the authorities in their day-to-day operations in handling these new and emerging COVID-19 specific scenarios~\cite{covid-vd, covid-vd-1, covid-vd-2}.
%Today, cameras are being deployed at city-scale throughout the world and different types of video analytics tasks are being performed on these video feeds as shown in Fig. \ref{fig:intro}. We refer to these video analytics tasks as Analytics Units (AUs). 

Depending on the video analytics task, cameras may be deployed either indoors or outdoors (Figure~\ref{fig:intro}. For example, video cameras for traffic analytics are deployed outdoors (pointing towards roads or highways), whereas for contactless fever screening of passengers disembarking from an airplane, the visual and thermal cameras are deployed indoors (pointing towards the boarding gates). Furthermore, for  the same video analytics task like video surveillance, cameras may be deployed indoors (in hallways inside a building) or outdoors (parking lots, for example). Clearly, different analytics tasks require different placements of video cameras and these cameras also view significantly different scenes. Also, depending on the environmental conditions, there may be natural lighting from the sun, artificial lighting or a combination of both. This can lead to bright or dark scenes and the lighting can vary over time (especially for outdoor locations) based on the weather conditions (cloudy, sunny, rainy, foggy, etc.) and time of the day (dawn, morning, afternoon, evening, dusk, twilight, night, etc.). 

Lighting can also vary in indoor locations depending on the placement of cameras and the  amount of artificial and natural light in that location. The particular direction of arrival of light can also change the way the scene is captured by the video camera due to projection of shadows. Different camera placements, applications and deployment conditions, as shown in Fig. \ref{fig:intro}, are just a few examples of many, dynamically changing factors that affect the accuracy of insights derived using video analytics. For real-time analytics and response, the accuracy of insights depends on the most recently observed video frames, whose quality and information content is directly impacted by the current camera parameter settings and ambient conditions near the camera. In this paper, we refer to a specific video analytics task as an {\it analytics unit} or AU. 
%~\figref{fig:intro} illustrates such a city-wide camera deployment, where different types of analytics tasks are being performed and each camera goes through different environmental changes throughout the day and across seasons as well.

%how video feeds from city-wide deployed camera captured experience different environment throughout the day, throughout different seasons even for different deployment areas.

%a.ka. knobs
%Cameras typically provide various configuration parameters a.k.a. knobs e.g. brightness, contrast, sharpness, color, gain, HDR, WDR, shutter speed, white balance, etc. to control the overall image quality that comes out of the camera. Some of them are software knobs while others are hardware knobs. Hardware knobs directly affect the way raw image is being captured, while software knobs affect the way the captured raw image is post processed before giving it out. 



%The final image produced by any camera depends on the type of camera lenses, camera modules and sensors, and also the overall Image Signal Processing (ISP) pipeline being used within the camera system \cite{5-min-guide}. ISP plays a crucial role in this and transforms the captured raw data into final compressed image. As part of this, several parameters are exposed to tune the final image quality. In this paper, we focus on a subset of these camera parameters to illustrate our techniques. The default settings provided by camera vendors do not work out-of-the-box in providing good image quality for different deployment conditions. For this, separate tuning and calibration step is provided by camera vendors. However, this manual tuning and calibration assumes that the conditions would remain more or less same, which, as mentioned before, is not the case. Therefore, there is a need to continuously tune these camera parameters so that high quality image can be produced by the ISP pipeline, which works well for AUs. Moreover, this needs to be done per camera at city-wide deployment scale, which is not practical for humans to do. $\approach$ addresses this need and automatically adjusts camera parameters to improve AU accuracy (for city-wide deployment scale). We leverage the fact that environmental changes are not sudden and happen gradually over a period of time, which enables $\approach$ to constantly monitor the conditions and adjust and fine tune dynamically as conditions change gradually. 

%This way $\approach$ adapts to the changing conditions, as we go, and avoid the situation where the camera starts producing frames which are extremely poor to perform highly accurate video analytics. 

%It is not practical for a human to keep adjusting these parameters, especially for city-scale deployment.

%There are two problems with this approach. \textit{First}, the conditions at the same location varies over time and one-time, single setting i.e. initial calibration does not work well over a period of time, as conditions change dynamically. Instead of initial calibration, we focus on the camera settings when it is in operation. \textit{Second}, manually tuning each individual camera for a city-wide deployment across different locations is tedious and not practical. Moreover, changing the settings and tuning for individual camera as the conditions change is impossible for humans to do.

%Real-time video analytics applications require that the quality of video feed coming in as input need to be good, so that accurate analytics can be performed. If this input video feed is of poor quality, which could be a result of improper camera settings for the specific conditions, then the accuracy of AU degrades significantly, (sometimes it even leads to falter the AU from detection or recognition). This degradation could have been avoided had the camera parameters been tuned to the specific conditions. In this paper, we address this problem and propose a novel technique to automatically and dynamically tune camera parameters as the conditions change over a period of time. We leverage the fact that these changes are not sudden and happen gradually over a period of time, which enables us to constantly monitor the conditions and adjust and fine tune dynamically as conditions change gradually. This way we adapt to the changing conditions, as we go, and avoid the situation where the camera starts producing frames which are extremely poor to perform highly accurate video analytics.


%\textcolor{red}{Quantatively mention if input video is of poor quality how much degradation occurs}\\



%Also, for PTZ cameras, knobs like ``Pan", ``Tilt" and ``Zoom" need to be continuously adjusted based on analytics requirement, as the object of interest moves in the scene.

Recognizing that a single, fixed setting of camera parameter values is inadequate to ensure consistent, high quality sensor output when environmental conditions change, we propose $\approach$. It is an automatic and dynamic system that adjusts to changing environmental conditions by suitably modifying the values of the configurable camera parameters. The modified settings result in higher quality sensor output, which in turn results in more accurate insights from machine learning models that process the sensor data. $\approach$ includes two important components. \textit{First}, an analytics quality estimator, which is a deep-learning model to automatically estimate the quality of insights from an analytics unit. As the environmental conditions around a sensor change, any change in accuracy of insights from the analytics unit is automatically detected by the AU-specific analytics quality estimator. Since different quality evaluation methods are typically used to estimate the quality of insights from different analytics units (this is described in Section~\ref{sec:AU-specific}), our quality estimator is AU-specific. However, our approach to design the quality estimator can be used to derive different AU-specific estimators (we present AU-specific analytics quality estimators for three different types of analytics units). \textit{Second}, a Reinforcement Learning (RL) module, which reacts to the changes in quality, as perceived by the quality estimator, and %reinforcement learner learns a model to 
automatically adjust the camera parameters to enhance the quality of insights (described in Section~\ref{camera-parameters-tuning}).

Training the reinforcement learner from scratch by using a real camera setup can be time-consuming because (a) we have to wait until the real camera observes different environmental conditions (b) we can process the frames only at the speed at which they are produced by the real camera e.g. 25 to 30 FPS and (c) for every action taken by the RL agent, depending on the camera, it can take 200-500 ms to change the camera parameter settings using APIs provided by the camera-vendor. To reduce the training time by an order of magnitude, we propose two virtual models to mimic the essential behavior of the camera: we design {\it virtual knobs} that can be set to different values to mimic the effects of assigning different values to the camera's configurable parameters, and we design a {\it virtual camera} model that mimics the output from a video camera at different times of the day. The virtual knobs model (described in Section \ref{virtual-knob}) allows the application of different camera parameter settings to the same input scene (something that is not possible to do with the real camera because only one set of camera parameter values can be in effect at any given time). 

The virtual camera model (described in Section~\ref{sec:vc-sim}) allows re-rendering of any video sequence for different environmental conditions. This is especially useful to quickly train the reinforcement learning model because multiple versions of a video sequence with known ground truth can be quickly rendered for different environmental conditions. Again, such a re-rendering of the same video scene for different environmental conditions is not possible with a real camera. Besides, with the help of virtual camera, we can process frames at a much faster rate, even upto 300 FPS by using more computing hardware. Using the virtual camera model, days worth of videos can be processed within hours. Also, for the RL agent, each action can be performed within 10s of milliseconds by using virtual knobs, which otherwise would take hundreds of milliseconds with real cameras. By combining these characteristics of the virtual models, where (a) we can render various environmental conditions (b) process frames at much higher speed and (c) take actions very quickly, we can train the RL module significantly faster (greater than 10x speedup).

%Training the reinforcement learner from scratch by using a real camera setup can be time-consuming (depending on the camera, it can take 200-500 ms to change the camera parameter settings using APIs provided by the camera-vendor). To reduce the training time by an order of magnitude, we propose two virtual models to mimic the essential behavior of the camera: we design {\it virtual knobs} that can be set to different values to mimic the effects of assigning different values to the camera's configurable parameters, and we design a {\it virtual camera} model that mimics the output from a video camera at different times of the day. The virtual knobs model (described in Section \ref{virtual-knob}) allows the application of different camera parameter settings to the same input scene (something that is not possible to do with the real camera because only one set of camera parameter values can be in effect at any given time). The virtual camera model (described in Section~\ref{alg:vc-sim}) allows re-rendering of any video sequence for different environmental conditions. This is especially useful to quickly train the reinforcement learning model because multiple versions of a video sequence with known ground truth can be quickly rendered for different environmental conditions. Again, such a re-rendering of the same video scene for different environmental conditions is not possible with a real camera.  

We train the proposed reinforcement learning module using a system consisting of the virtual camera, virtual knobs, the analytics unit, and its quality estimator. After such training, the reinforcement model is deployed and continuously fine-tuned in the real deployment by using video data from the real camera. $\approach$ can be used to automatically create and fine-tune reinforcement learning models for thousands of cameras in large-scale deployments like city-wide surveillance systems.


In this paper, we make the following contributions:
\begin{enumerate}
%\vspace{-0.5in}
    \item We empirically show that a fixed set of values for the camera parameters does not lead to consistent, high-quality insights as environmental conditions change. Rather, the desirable camera setting varies as environmental conditions change. Also, the desired camera parameter setting varies across different analytics units for the same environmental conditions. This motivates the need for automatic and dynamic adjustment of camera parameters as analytics tasks and environmental conditions change.
    %are not adjusted based on the environmental conditions,  then different AUs suffer with different levels of deterioration. We then show that there exists a better camera parameter setting that can improve AUs performance.
    
    %\item We show empirically that due to change in environmental conditions throughout the day, the performance of different AUs deteriorate differently on the captured frames from same camera feed while camera is kept at a constant default setting. We then show that there exists a better camera parameter setting that can improve the AU performance.
    
    \item We propose a new methodology to design \emph{AU-specific Analytics Quality Estimator}, and we design quality estimators for three different analytics units (face recognition, person detection and face detection).
    
    \item We propose a reinforcement learning method to automatically, and dynamically tune the configurable parameters of a complex sensor to yield consistent, high-quality insights. To our knowledge, this is the {\it first} approach to automatically, and dynamically tune camera parameters to enhance specific analytics tasks. 
    
    \item To significantly speed-up reinforcement learning, we propose virtual knobs and virtual camera models that mimic essential characteristics of a camera; these virtual models are used in reinforcement learning in lieu of a real camera to quickly learn a good reinforcement learning model, and the learnt model is fine-tuned using a real camera in a real-world deployment. Our dynamic tuning approach results in up to 12\% improvement in the accuracy of insights from several video analytics tasks.
    
    
 %   \item We introduce a new mechanism to find digital equivalence for camera parameters, called as \emph{virtual knob}, which enables us to study performance of AUs under different camera settings.
    
    %\item We introduce a \emph{new} mechanism, \emph{digital twin} that finds the digital equivalence of physical camera parameters. \emph{digital-Twin} enables us to study the impact of various camera settings on same scene and observe the AU performance consistently under continuous scene change. 
    
%    \item We validate that for an AU, the best camera setting is different for different environmental conditions, thereby motivating the need for automatic and dynamic adjustment.
    
    %\item We also validate that the possible best camera parameter settings for different images and video-snippets (i.e., captured under various environmental conditions) are different while parameter value varies in same range in digital domain obtained from \emph{digital twin}.
    
   % \item We propose a State-Action-Reward-State-Action (SARSA) Reinforcement Learning (RL) algorithm to dynamically adapt to changing environmental conditions and as part of this, we propose a \emph{new policy} for the agent to take actions and learn to maximize the reward.
    
    %\item We propose a State-Action-Reward-State-Action (SARSA) reinforcement learning (RL) algorithm to tune the camera with the best possible parameter setting while adapting towards different environmental conditions. We introduce a \emph{new policy} that helps SARSA RL agent to choose an appropriate action from current state.
    
  %  \item We propose a \emph{new} \emph{virtual-camera (VC) simulator}, which enables us to apply various environmental characteristics and study impact of various camera settings on exact same scene, and also allows us to rapidly train and test RL algorithms for automatic camera parameter tuning. 
    
    %\item We propose a \emph{new} \emph{virtual-camera (VC) simulator} which loops through pre-recorded video and can simulate various scene characteristics for different time of day according to actual physical camera without changing the scene content. \emph{VC simulator} design also helps to train RL faster with various reward functions and various actions can be tried on exact scene in realtime. 
    
 %   \item During runtime, RL needs continuous and automatic reward for every action it takes. We first observe that SOTA AQuA-filter~\cite{paul2021aqua} can't provide fine-grained quality evaluation for different AUs. To address this, we define a \emph{new Analytic Quality (AQ)} metric, specific for each AU, and using that metric, we train AU-specific AQuA-classifier, which provides quality reward for every RL action.
    
    %\item During runtime, RL needs continuous and automatic reward for every action i.e. parameter setting, it takes. We first observe that SOTA AQuA-filter~\cite{paul2021aqua} can't provide fine-grained quality evaluation for different AUs. We define \emph{new Analytic Quality (AQ)} metric specific for each AU, and using that metric, we train AU-specific AQuA-classifier that provides quality reward for every RL action.
    
%    \item We conduct multiple evaluations that show efficacy of different components used within $\approach$.
    
    %\item We conduct multiple evaluations that show efficacy of different $\approach$'s components. 
    
 %   \item To the best of our knowledge, $\approach$ is the \emph{first system} that adapts to changing environmental conditions by automatically tuning camera parameters based on the need of specific AU and improves the accuracy of AUs.
    
    %\item To the best of our knowledge, $\approach$ is the \emph{first system} that devises the methodology to automatically and dynamically tune the actual physical camera sensor parameters adapting to different environment and also based on various analytic unit perception.
    
    
\end{enumerate}

%The real-world deployment of $\approach$ with two side-by-side cameras, shows that $\approach$ can provide 11\% accuracy improvement without impacting latency of analytical pipeline.

%while tuning the four popular camera parameters.

%<Describe contributions and organization of the paper>

%Introduce the problem - In a city wide deployment e.g. 100 cameras, the conditions seen by each camera is different and it changes during the course of the day, week and even across months, as the season changes. All these changes however are gradual and different for each camera. A single camera setting for all these city-wide deployed cameras is inadequate. Changing them individually is impractical as each one requires different settings based on the scene the camera is observing. We have an opportunity to automatically monitor and tune camera settings for each camera individually, so that AU accuracy is kept intact. 

%Introduce the problem - cameras can have only one setting and typically it is tuned based on human perception. However, AUs can obtain better results with different camera settings. Thus, there is a disconnect and there is a need for automatic camera parameters tuning to improve AUs accuracy. 
%Moreover, multiple AUs can run on the same camera stream and each AU might need different camera settings. Introduce digital twin concept here and that software based digital transformations can help in these scenarios.

==> oldfiles/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/processing-pipeline.png}
    %\vspace{-0.2in}
    %\caption{Processing pipeline in camera}
    \caption{$\approach$ Overview}
    \label{fig:pipeline}
    %\vspace{-0.3in}
\end{figure}
%\vspace{-0.2in}

%\subsection{Environmental effect} 

\figref{fig:pipeline} shows the processing pipeline within a camera. 
Photons from the external world reach the image sensor through an optical lens. The image sensor  uses a bayer filter~\cite{bayer1976color} to create the raw-image data, which is further enhanced by a variety of image processing techniques~\cite{ramanath2005color} like  demosaicing, denoising, white-balance, color-correction, sharpening and image compression (JPEG/PNG or video compression using H.264~\cite{x264}, VP9~\cite{vp9}, MJPEG, etc.) before the image or video is retrieved from the camera. The camera manufacturer exposes many parameters  that can be set to control the image generation process. To illustrate the proposed dynamic tuning approach,  we consider four popular parameters that are common to almost all cameras: brightness, contrast, color-saturation (a.k.a colorfulness) and sharpness. Please note that other camera parameters can also be dynamically tuned using the $\approach$ system.

\if 0
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/day-night-improv.PNG}
    %\vspace{-0.2in}
    %\caption{Processing pipeline in camera}
    \caption{Parameter Tuning for various Environment}
    \label{fig:cam-param-tuning-env}
    %\vspace{-0.3in}
\end{figure}

\begin{table}[h!]
\begin{tabular}{|c|c|c|}
    \hline
    Environment & Parameter & AQ\\
    & Setting & Score\\
    \hline
    \multirow{2}{*}{DAY} & (default) [50,50,50,50]  & 0.82  \\
    \cline{2-3}
    & (best) [80,80,60,40]  & 0.85 \\
    \hline
    \multirow{2}{*}{NIGHT} & (default) [50,50,50,50]  & 0.43  \\
    \cline{2-3}
    & (best) [100,90,30,70]  & 0.59 \\
    \hline
\end{tabular}
\caption{Best Camera Parameters for Different Environments}
\label{tab:cam-param-tuning-env}
 \vspace{-0.3in}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/setting-vs-postprocess.PNG}
    %\vspace{-0.2in}
    %\caption{Processing pipeline in camera}
    \caption{Parameter Tuning vs Post-processing}
    \label{fig:param-tune-vs-postprocess}
    %\vspace{-0.3in}
\end{figure}
\fi








Environmental conditions do change during a day, and these changes affect the quality of images and videos retrieved from the camera.
%induce various distortions in the frame during acquisition (i.e., over-exposure in presence of sunlight, low-light noise and under-exposure during night-time etc.). These distortions, in turn, affect and most of the time, deteriorate AU performance, if no changes are done to camera settings as conditions change.
%show environmental effect on face and person detection
There are no publicly available video datasets that capture the environmental variations in a day by using the same camera (and location). Therefore, we use several videos from our customers to study the impact of these variations on image quality and the insights derived. These videos were captured by camera that was stationary, and the field of view was fixed for the entire length of video capture. 
%These videos were obtained by using taken outside a baseball stadium by single camera from morning to evening~\footnote{These are confidential customer videos, and hence we cannot share the dataset as of now.}. 
For these videos, we also have labelled ground-truth information for several analytics tasks like face detection and people detection. We use RetinaNet~\cite{deng2019retinaface} to detect faces, and EfficientDet-v8~\cite{tan2020efficientdet} to detect persons. In both cases, we compare the analytics results with the ground truth information to measure the accuracy of insights from the AUs (we compute the mean Average Precision, or mAP, by using pycocotools~\cite{pycoco}).

%Under default camera settings, figure~\ref{fig:daylong_face_det} and ~\ref{fig:daylong_person_det} show that 
\figref{fig:face_person_env}(a) shows the mAP values for the face detection AU during four different times of the day: morning, noon, afternoon, and evening. For the default camera parameter settings, we see that the mAP values vary as the day progresses (blue bars). Therefore, changes in environmental conditions do affect the quality of the frames retrieved from the camera, and this in turn affects the accuracy of insights that are derived from the video data. The green bars show the mAP values when we modify four virtual knobs (as explained in ~\secref{virtual-knob} and ~\secref{sec:knob-impact}) i.e. brightness, contrast, color-saturation and sharpness of each frame as the day progresses. In fact, for each frame, we exhaustively try all combinations of brightness, contrast, color-saturation and sharpness, and select the combination that yields the best analytics results. We use the best combination to modify the frame, and use this modified frame for analytics processing. As shown in the Figure, the mAP values for the green bars are higher than the mAP values for the default settings (blue bars).  We observe a similar trend in \figref{fig:face_person_env}(b) that shows the mAP values for the person detection AU.
We note that by varying the four parameters, we observe a 6.1-15.7 mAP improvement for face detection AU (\figref{fig:face_person_env}(a)). For the person detection AU, which tries to detect the whole person rather than just the face, we observe a  mAP improvement of 4.9-9.7 (\figref{fig:face_person_env}(b)).

Empirical data in \figref{fig:face_person_env} suggests that there is scope to tune the four camera parameters to improve the image capture process, and enhance the accuracy of insights derived. Now, to see this in action with a real camera, we simulate \emph{DAY} and \emph{NIGHT} condition in our lab and see the performance of face-recognition AU pipeline described in~\cite{schroff2015facenet}. In our setup, we use two sources of light and keep one of them always \emph{ON}, while the other one is manually turned \emph{ON} or \emph{OFF}. When both the light sources are \emph{ON}, it is bright, thereby simulating \emph{DAY} condition, while when one of them is \emph{OFF}, it is low-light, thereby simulating \emph{NIGHT} condition. We place face cutouts of 10 unique individuals in front of the camera and run face recognition pipeline which recognizes these faces. We run this pipeline for various camera settings and for different face matching threshold for the face recognition AU, and measure the \emph{Recall}~\footnote{This face-recognition AU is very good in telling apart face-images that are not of same person. Therefore, high precision is obtained and it remains almost same for different environments, and hence we focus only on Recall.} i.e. true-positive rate~\cite{roc}, which is a ratio of number of faces correctly recognized (true-positive) by the AU and the total number of faces in the ground truth. ~\figref{fig:recall_day} shows the Recall for \emph{DAY} condition for various thresholds, while ~\figref{fig:recall_night} shows the Recall for night condition for various thresholds. In both cases, the ``Default" settings is where the four camera parameters are set to the manufacture provided default values, while the ``Best" settings is obtained by programmatically changing the four camera parameters using VAPIX API~\cite{vapix} provided by camera vendor, and finding the setting that gives the highest Recall value. We vary each parameter from 0 to 100 in steps of 10 and capture frame for each camera setting. This gives us $\approx$14.6K frames for each condition i.e. \emph{DAY} and \emph{NIGHT}. To change one camera setting, it takes about $\sim$ 200 ms through VAPIX API and it took about \emph{7 hours} to capture the frames for each condition. We see that the Recall for ``Default" setting for \emph{DAY} condition goes down at higher thresholds, indicating that some faces were not recognized, whereas for \emph{NIGHT} condition, the Recall remains constant at a low value for all thresholds, indicating that some faces were not being recognized in the ``Default" setting. When we actually changed the camera parameters for both conditions and obtained the ``Best" setting, we see that we are able to achieve the highest Recall i.e. 1, indicating that all the faces are correctly recognized. This shows that it is indeed possible to improve AU accuracy by changing the four camera parameters. 

%create a scenario in our lab, where we place 10 face cut outs of 10 different individuals in front of a camera and simulated \emph{DAY} and \emph{NIGHT} condition by using two sources of light. First light source is always ON, while the second one is manually turned ON and OFF. When the second light source is ON, it is bright and simulates \emph{DAY} condition, while when it is OFF, it simulates low-light i.e. \emph{NIGHT} condition. We use face-recognition AU pipeline described in~\cite{schroff2015facenet} that recognizes faces from 10 unique face cutouts placed in front of the camera. 

%\textcolor{blue}{To find out the possible accuracy enhancement quantitatively, we use face-recognition AU pipeline described in~\cite{schroff2015facenet} that recognizes faces from 10 unique face cutouts placed in front of the camera. We simulated two different environmental conditions inside lab. Keeping all light-bulbs on simulates the \emph{DAY} environment while low-light condition with all light-bulbs off creates \emph{NIGHT} condition.
%We vary four popular camera parameters from 0 to 100 at a step of 10 using VAPIX API~\cite{vapix} provided by camera vendor. It takes $\sim$ 200 ms to change each camera parameter setting. For each environment, it takes \emph{7 hours} to capture frames ($\approx$14.6K) for all possible camera settings. 
%Face-recognition AU determines if an input face image matches with any image in a pre-defined gallery of face images for a given matching threshold. We measure the accuracy of the insights obtained from face-recognition AU in terms of \emph{Recall}~\footnote{Since, this face-recognition AU is very good in telling apart face-images that are not of same person. Hence, high precision is obtained and it remains almost same for different environments.}  (i.e., true-positive rate) ~\cite{roc} for different matching thresholds. Higher recall shows how accurately AU can recognize relevant faces providing a matching score higher than threshold.
%The best camera parameter setting can improves the recall for both night and day environment, also shown in~\figref{fig:recall-phy}.}

Please note that modifying camera parameters to capture a better image is fundamentally different from applying transformations on the frames retrieved from the camera. For example, if the image captured by the camera is sufficiently poor due to sub-optimal camera settings, then no further transformations of the video stream from the camera can improve the accuracy of analytics. As shown in ~\figref{fig:param-tune-vs-postprocess}, we intentionally changed the default camera parameters to certain sub-optimal settings denoted by S1, S2, S3 and S4 and measured the Recall for face recognition AU as before. In these settings, the frames from the camera are of poor quality and we show the Recall for various thresholds, which is quite low for all the settings. Then, we apply digital transformation on these using virtual knobs (as explained in ~\secref{virtual-knob} and ~\secref{sec:knob-impact}) and note the highest Recall value that we can obtain. We see that the Recall improved, compared to the original setting, but it is still quite low.
%\textcolor{blue}{For this, we capture the frames captured with four different suboptimal settings under \emph{NIGHT} condition (i.e., simulated inside the lab) and digitally augment those with various virtual knob values of those four camera parameters (explained in~\secref{sec:knob-impact}). ~\figref{fig:param-tune-vs-postprocess} presents that although digital postprocessing after frame acquisition improves recall, it always provide inferior accuracy (i.e., recall) to the best camera setting.} 
This is because, due to the sub-optimal camera settings, the frames from the camera do not have adequate information about the scene being captured. Now, if we directly change the actual camera parameters, shown by ``Best setting", then we are able to achieve the highest Recall i.e. 1. Since we are already achieving the highest possible Recall value, applying further digital transformation on this will not help any further. This shows that modifying camera parameters is fundamentally different from applying transformations on the frames retrieved from the camera. 

%\textcolor{blue}{Since, recall under best camera setting is already high, applying further digital postprocessing does not improve the analytics accuracy}


%on each frame of the videoif we dynamically modify the camera parameters in response to changing environmental conditions. This experiment 

%shows the AU accuracy for videos taken from same camera under default camera settings varies throughout the day due to presence of different environmental conditions, as shown in ~\figref{fig:face_person_env}. Specifically, during noon (in-presence of glaring sunlight), the captured faces inside the frame, get over-exposed, hence result in lower accuracy than the AU performance for the morning-time video. However, evening-time video suffers from low-light noise, which also results in accuracy degradation. Faces in intermediate \textit{afternoon video}-frames get slightly occluded which makes detection difficult for face-detector, but due to better lighting conditions during afternoon, person-detector AU can accurately predict the bounding-boxes, results in the best mAP performance.



%For face detection AU, the maximum improvement is observed for noon-time video, while best-parameter setting impacts evening-time video the least. 
\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.25 in]{figs/fd-performance.png}
    \caption{Face Detection}
    \label{fig:daylong_face_det}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.25 in]{figs/person-performance.png}
    \caption{Person Detection}
    \label{fig:daylong_person_det}
\end{subfigure}
 \caption{AU performance variation in a day}
  \label{fig:face_person_env}
 \vspace{-0.2in}
\end{figure}

\if 0
\begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[Face detection]{\includegraphics[width=4cm]{figs/fd-performance.png}\label{fig:daylong_face_det}}
 & \subfloat[Person detection]{\includegraphics[width=4cm]{figs/person-performance.png}\label{fig:daylong_person_det}
 }
 \end{tabular}
 \end{tabularx}
 \caption{AU performance variation in a day}
  \label{fig:face_person_env}
 \end{figure}
 \fi
 
 
%\if 0
 \begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.1 in]{figs/recall_day_excel_1.png}
    \caption{DAY}
    \label{fig:recall_day}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.1 in]{figs/recall_night_excel_1.png}
    \caption{NIGHT}
    \label{fig:recall_night}
\end{subfigure}
 \caption{Parameter Tuning Impact for Face-recognition AU}
  \label{fig:recall-phy}
 \vspace{-0.2in}
\end{figure}
%\fi
 
 
 \if 0
 \begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[DAY]{\includegraphics[width=4cm]{figs/recall_day_excel_1.png}\label{fig:recall_day}}
 & \subfloat[NIGHT]{\includegraphics[width=4cm]{figs/recall_night_excel_1.png}\label{fig:recall_night}
 }
 
 \end{tabular}
 \end{tabularx}
 \caption{Parameter Tuning Impact for Face-recognition AU}
  \label{fig:recall-phy}
 \end{figure}
 \fi
 
 \begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_1_excel_1.png}
    \caption{Suboptimal Setting-1 (S1)}
    \label{fig:recall_night_1}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_2_excel_1.png}
    \caption{Suboptimal Setting-2 (S2)}
    \label{fig:recall_night_2}
\end{subfigure}
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_3_excel_1.png}
    \caption{Suboptimal Setting-3 (S3)}
    \label{fig:recall_night_3}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_4_excel_1.png}
    \caption{Suboptimal Setting-4 (S4)}
    \label{fig:recall_night_4}
\end{subfigure}
 \caption{\textit{Parameter Tuning} vs \textit{Postprocessing} for \emph{NIGHT}}
  \label{fig:param-tune-vs-postprocess}
 \vspace{-0.2in}
\end{figure}
 
 

\if 0 
\begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[Suboptimal Setting-1 (S1)]{\includegraphics[width=4cm]{figs/recall_night_1_excel_1.png}\label{fig:recall_night_1}}
 & \subfloat[Suboptimal Setting-2 (S2)]{\includegraphics[width=4cm]{figs/recall_night_2_excel_1.png}\label{fig:recall_night_2}
 }\\
  \subfloat[Suboptimal Setting-3 (S3)]{\includegraphics[width=4cm]{figs/recall_night_3_excel_1.png}\label{fig:recall_night_3}}
 & \subfloat[Suboptimal Setting-4 (S4)]{\includegraphics[width=4cm]{figs/recall_night_4_excel_1.png}\label{fig:recall_night_4}
 }
 
 \end{tabular}
 \end{tabularx}
 \caption{\textit{Parameter Tuning} vs \textit{Postprocessing} for \emph{NIGHT}}
  \label{fig:param-tune-vs-postprocess}
 \end{figure}
 \fi


%\emph{Analytical Quality (AQ)} score for the face-recognition application is defined as harmonic mean of average positive match-scores (i.e., score between detected face and its corresponding gallery image), average negative match-scores (i.e., maximum score between detected face and with any other gallery image) and number of detected faces. The AQ score (i.e., ranges from 0 to 1) provides high quality values when high matching score between corresponding faces from detections and ground-truth and low matching score between detected faces with faces of other people is obtained with more number of faces from ground-truth are detected.  

%~\tabref{tab:cam-param-tuning-env} shows best camera parameter settings (i.e., that provides best AQ score) are different for different environment. 
%\textcolor{blue}{~\figref{fig:recall-phy} also shows that best camera parameter setting can improves the recall for both night and day environment. While for \emph{DAY}, due to proper lighting conditions, recall under default condition is high hence improvement is less but \emph{NIGHT}-time video experiences a higher improvement under best parameter setting than the default one due to elimination of low-light noises in the captured frame. }

%\textcolor{blue}{we take the frames captured under different settings under \emph{NIGHT} condition and digitally augment those with various virtual knob values of those four camera parameters (explained in~\secref{sec:knob-impact}). ~\figref{fig:param-tune-vs-postprocess} presents that postprocessing after frame acquisition always improves recall. While ~\figref{fig:recall_night} presents that postprocessing provides similar improvement as the best camera parameter setting but if camera has already applied some irreversible and lossy processing, then directly tuning the camera parameters can only provide the maximum recall improvement as shown in ~\figref{fig:recall_night_1}~\ref{fig:recall_night_2}~\ref{fig:recall_night_3} for three different initial camera parameter setting.  ~\figref{fig:recall_night} also shows that postprocessing can't provide much benefit on top of frames captured under best camera parameter tuned according to the external environment.}


\if 0
\textcolor{red}{Show example of proprietary frames to validate the problem?}
\textcolor{blue}{If it is okay, we can show frames during day time and night time, but with no person in the frame (to avoid revealing any personally identifiable information) - not sure if even this is allowed. If we can't add even such frames, then maybe add example from public dataset showing such frames and mention that this is an example and not from our actual confidential dataset.}
\fi
 

 
 
 
 


==> oldfiles/motivation_1.tex <==
\section{Motivation}
\label{section:motivation}

In this section, we motivate the need for automatic dynamic camera setting 
by experimentally showing the impact of environment change on AU accuracy under the
same camera setting and the impact of camera settings on AU accuracy 
under the same environment condition.

\subsection{Effect of Environment Change on AU Accuracy}
\label{subsec:environ}

Environmental conditions change over time, and these changes affect
the quality of images and videos retrieved from a surveillance
camera. Environmental changes happen for at least three reasons.
First, it can be induced due to change of
the Sun's movement throughout a day, \eg sunrise and sunset.
Second, it can be triggered by 
% changes in a longer time scale than a day
% due to dynamic change in sun position, various 
changes in weather conditions, \eg rain, fog, and snow.
Third, even for the same weather condition at exactly the same
time of the day, in different 
deployment sites, \eg parking lot, factory, shopping mall, and airport,
the videos captured by the cameras can have diverse content and lighting conditions.

To illustrate the impact of environment changes on image quality and
consequently on the accuracy of AUs, we experimentally measure the
accuracy of two popular AUs, face detection and person detection,
throughout a 24-hour one-day period.  Since there are
no publicly available video datasets that capture the environmental
variations in a day by using the same camera (and location), we use
several proprietary videos from our customers. Specifically, the videos
in our dataset were captured outside a baseball stadium by a
stationary camera, the field of view (FoV) was fixed for the
entire duration of video capture, and we have
labeled ground-truth information for several analytics tasks
including face detection and people detection.

We use RetinaNet~\cite{deng2019retinaface} for face detection, and
EfficientDet-v8~\cite{tan2020efficientdet} for person detection. In both
cases, we compare the analytics results with the ground truth
information to measure the accuracy of insights from the AUs.  We
compute the mean Average Precision (mAP) by using pycocotools~\cite{pycoco}.

\figref{fig:daylong_face_det} shows the average mAP values for the
face detection AU during four different time periods of the day:
{morning (8AM - 10AM), noon (12PM - 2PM), afternoon (3PM -
  5PM), and evening (6PM - 8PM)} under the default camera parameter
settings vary by up to 40\% as the day progresses (blue bars).
Similarly, \figref{fig:daylong_person_det} shows that the average mAP
values for the person detection AU under the default camera parameter
settings vary by up to 24\% during the four time periods.
These results show that changes in environmental
conditions can affect the quality of the frames retrieved from the
camera and consequently the accuracy of the insights that are
derived from the video data. 


\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.25 in]{figs/fd-performance.png}
    \caption{Face Detection}
    \label{fig:daylong_face_det}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.25 in]{figs/person-performance.png}
    \caption{Person Detection}
    \label{fig:daylong_person_det}
\end{subfigure}
 \caption{AU accuracy variation in a day and impact of camera settings.}
  \label{fig:face_person_env}
 \vspace{-0.2in}
\end{figure}



\subsection{Impact of Camera Settings on AU Accuracy}
\label{subsec:impactofsettings}

To illustrate the impact of camera settings on AU accuracy, we
consider four popular parameters that are common to almost all
cameras: {\em brightness, contrast, color-saturation} (a.k.a
colorfulness), and {\em sharpness}.
%   We note that other
%   camera parameters can also be dynamically tuned using the $\approach$
%   system. 

\textbf{Methodology:} Analyzing the impact of camera settings on video
analytics faces a significant challenge: it requires applying
different camera parameter settings to the same input scene and
measuring the resulting accuracy of an AU. The
straight-forward approach is to use multiple cameras with different
camera parameter settings to record the same input scene. However,
this approach is impractical as there are thousands of different
combinations of even just the four camera parameters we consider.  To
overcome the challenge, we proceed with two workarounds.  First, we
will show the impact of camera settings on a stationary scene
with a real camera.  Second, we develop {\em virtual camera knobs}
which are digital equivalents of camera parameters, and then use
virtual knobs to analyze the impact of camera settings on small video
snippets, \ie groups of frames.

\textbf{Experiment 1: using a real-camera.} To see the impact of
camera settings in action with a real camera, we simulate {DAY} and
{NIGHT} conditions in our lab and evaluate the performance of
a face-recognition AU, Neoface-v3~\cite{NIST}\footnote{
  This face-recognition AU is ranked first in the world in the most
  recent face-recognition technology benchmarking by NIST.}. 
We use two sources of light and keep one of them always
\emph{ON}, while the other one is manually turned \emph{ON} or
\emph{OFF}. When both light sources are \emph{ON}, it is bright,
thereby simulating the {DAY} condition; when one of them is
\emph{OFF}, it is low-light, thereby simulating the {NIGHT}
condition. 

We place face cutouts of 10 unique individuals in front of
the camera and run the face recognition pipeline to recognize these
faces. We run this pipeline for various camera settings and for
different face matching threshold for the face recognition AU.
{Since this face-recognition AU is very
  good at telling apart face-images that are not of the same
  person and hence has high precision despite 
 environment changes, we focus on measuring Recall,
% and measure the \emph{Recall}
\ie true-positive rate,
% ~\cite{roc}, 
which is the ratio of the number of
faces correctly recognized (true-positive) by the AU and the total
number of faces in the ground truth. 
%
We compare AU results under the ``Default" camera settings,
\ie the default
values provided by the manufacturer,
and ``Best'' settings for the four camera parameters.
% The ``Default'' settings  are from the manufacturer provided default values.
To find the ``Best'' settings, we 
% programmatically
change the four camera parameters using the VAPIX API~\cite{vapix}
provided by the camera vendor to find the setting that gives the
highest Recall value. 
%
Specifically, we vary each parameter from 0 to 100 in steps of
10 and capture the frame for each camera setting. This gives us
$\approx$14.6K (11$^4$) frames 
for each condition.
%
To change one camera setting, it takes about 200
ms through the VAPIX API and in total it took about \emph{7 hours} to capture the
frames for each condition. 

~\figref{fig:recall_day} shows the Recall for the {DAY} condition
for various thresholds and ~\figref{fig:recall_night} shows the Recall
for the NIGHT condition for various thresholds.
%
We see that under the ``Default''
settings, the Recall for the \emph{DAY} condition goes down at higher thresholds,
indicating that some faces were not recognized, whereas for
the {NIGHT} condition, the Recall remains constant at a low value for
all thresholds, indicating that some faces were not being recognized
regardless of the face matching thresholds.
%
In contrast, when we changed the camera parameters for both conditions to the
``Best" settings, the AU achieves the highest Recall, 100\%,
indicating that all the faces are correctly recognized. These results
show that it is indeed possible to improve AU accuracy by adjusting
the four camera parameters.


\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.1 in]{figs/recall_day_excel_1.png}
    \caption{DAY}
    \label{fig:recall_day}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.1 in]{figs/recall_night_excel_1.png}
    \caption{NIGHT}
    \label{fig:recall_night}
\end{subfigure}
 \caption{Parameter Tuning Impact for Face-recognition AU}
  \label{fig:recall-phy}
 \vspace{-0.2in}
\end{figure}


%define virtual knobs and impacts

\paragraph{Experiment 2: using virtual knobs.}
{\em Virtual knobs} are digital equivalent of {camera
parameters of the image processing stage in ~\figref{fig:pipeline}}. 
\comment{Given a frame taken under the mid-values of camera setting ranges,
transforming the frame using a set of virtual knobs $v_i$
will result in a new frame identical
or very similar to a frame capture of the same scene using the real camera
under a different set of camera settings $s_i$.
}

To establish the mapping between a given set of camera settings and
the equivalent virtual knobs $v_i$, we use a \textit{AXIS Q1615}
camera and an image transformation algorithm in the Python Imaging
Library~\cite{pil}.
%  Algorithm~\ref{alg:digital-twin} describes our method
%  for establishing the mapping between parameter values of the image
%  transformation algorithm (which are the virtual knobs) and camera
%  parameter values. 
%
First, we set the camera parameters to their mid-range, or
as recommended by the camera manufacturer, and we capture an image
$im$. Then we progressively change the parameter value of each camera parameter
% (shown in the outer loop of Algorithm~\ref{alg:digital-twin}) 
through the range of values supported by the camera vendor 
to generate different images $im_p$ for the same static scene. 
%
Next, for each image $im_p$, 
% which corresponds to a particular camera parameter setting, 
% the inner loop 
we determine the closest set of
parameter values of the image transformation algorithm that will
produce a modified image $im_d$ from image $im$ that
has the same {or closest} image quality as $im_p$.
%
This set of parameter values of the image transformation
algorithm form the virtual knob values that correspond to the specific
camera parameter settings that generated image $im_p$.  
%
%   In this way, the above procedure derives the correspondence between
%   different camera parameter settings and the different parameter values
%   of the image transformation algorithm (\ie virtual knob values). 
%
We use a de-facto full-reference image-quality assessment metric, structural similarity
(\textit{SSIM})~\cite{ssim}, to match the image quality of $im_p$
% (image from camera) 
and $im_d$.
% (modified image produced by the image transformation algorithm). 
For example, if the SSIM value for the pair
($im_p$, $im_d$) is higher than 0.9, the image from the camera
and the modified image from the image transformation algorithm are
{considered sufficiently similar~\cite{cuervo2015kahawai}.}
% both of good visual quality

Since virtual knobs can transform a video as if it were recorded using
a different set of camera settings, they provide a convenient way of
evaluating the impact of camera settings on the accuracy of AUs on
camera feeds without using many physical cameras, by using a recorded video.

%  they allow us to to study the impact of 
%  camera settings directly using recorded videos.
%

We consider 19 video snippets from the HMDB dataset~\cite{Kuehne11}
and 11 video snippets from the Olympics
dataset~\cite{niebles2010modeling}. Using cvat-tool~\cite{cvat}, we
manually annotated the face and person bounding boxes which forms our
ground truth.  Each video-snippet contains no more than a few hundred
frames, and the environmental conditions for a video are largely
constant. However, the environmental conditions appear
to vary across the video snippets \comment{due to change in
  video capture locations}. We determine a single best combination of
virtual knobs for each video, \ie one that results in the highest
analytical quality for that video.
%
\figref{fig:hmdb51} and \figref{fig:olympics} show the distribution of
the best virtual knob combinations for the videos in the two datasets,
respectively. We see that with a few exceptions, the best virtual knob
combinations for different videos in a dataset do not cluster,
suggesting that any fixed camera parameter setting will not be ideal for
different environmental conditions or analytics tasks.


%    We note that by varying the four parameters, we observe a 6.1-15.7 mAP
%    improvement for face detection AU performance on day-long video
%    segments (\figref{fig:daylong_face_det}). Similarly for the person
%    detection AU, which tries to detect the whole person rather than just
%    the face, we observe a mAP improvement of 4.9-9.7
%    (\figref{fig:daylong_person_det}). 

Finally,
going back to the experiments in \S\ref{subsec:environ}, for
  the face detection and person detection AUs, we 
\comment{sampled ????? frames from the the day-long video,}
and for each sampled frame,
we exhaustively tried all combinations of
 the four camera parameter values using virtual knobs, and selected the
combination that yields the best analytics result for that frame.
The resulting average mAP values from using these ``optimal''
per-frame camera settings for the four camera parameters 
% (brightness, contrast, color-saturation and sharpness) 
as the day progresses 
for the two AUs are shown in the green bars in 
\figref{fig:daylong_face_det}
and \figref{fig:daylong_person_det}, respectively.
%   We use the best combination to modify the
%   frame, and use this modified frame for analytics processing. 
We see that for face detection the average mAP values for
the optimal settings are 6.1\% -- 15.7\% higher than for
the default settings, and for person detection the average mAP values 
under optimal settings are 4.9\% -- 9.7\% higher than 
under the default settings.
%
These results suggest that the impact of environment 
on the accuracy of AUs can be remedied
by tuning the four camera parameters to improve the image capture
process.  
}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/hmdb51_face.pdf}
    \caption{Face Detection}
    \label{fig:hmdb_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/hmdb51_person.pdf}
    \caption{Person Detection}
    \label{fig:hmdb51_person}
\end{subfigure}
\caption{Distribution of best configurations for two AUs on \emph{HMDB} video snippets}
\label{fig:hmdb51}
 \vspace{-0.2in}
\end{figure}

\begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/olympics_face.pdf}
    \caption{Face Detection}
    \label{fig:olympics_face}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.3 in]{figs/olympics_person.pdf}
    \caption{Person Detection}
    \label{fig:olympics_person}
\end{subfigure}
\caption{Distribution of best configurations for two AUs on \emph{Olympics} video snippets}
\label{fig:olympics}
\end{figure}

\begin{table}[h!]
\caption{Best configuration Accuracy Improvement}
\label{tab:best-video-conf}
{
\small
\begin{tabular}{||c|c||c|c|c|}
    \hline
    Video-Dataset & AU & \multicolumn{2}{c|}{mAP}\\
    & & \multicolumn{2}{c|}{improvement}\\
    \cline{3-4}
    & & Max & Mean \\
    \hline
    \multirow{2}{*}{Olympics} & Face Detection  & 19.23 & 1.68  \\
    \cline{2-4}
    & Person Detection & 40.38 & 8.38 \\
    \hline
    \multirow{2}{*}{HMDB} & Face Detection  & 18.75 & 4.22  \\
    \cline{2-4}
    & Person Detection & 57.59 & 12.63 \\
    \hline
\end{tabular}
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Post-processing Is not Enough} 
\label{subsec:notrnough}

\if 0
\textcolor{red}{Existing works~\cite{???} assume that a camera
  platform only exposes stream endpoints (\eg rtsp and url) to
  vision applications and applies necessary transformations on the
  frames acquired from the camera to improve the performance of the
  vision applications.} 
\fi

It is important to note that modifying camera parameters to capture a
better image or video feed is fundamentally different from applying transformations
to the frames already retrieved from the camera,
which has been previously 
used to optimize the resources for delivering the video over the Internet,
\eg \cite{201465, jiang2018chameleon}.
%
In particular, if the image
captured by the camera is sufficiently poor due to sub-optimal camera
settings, then no transformations of the video stream from the
camera can improve the accuracy of analytics. 
%
To see this, we repeated the same face-recognition AU experiment with a
real camera in \S\ref{subsec:impactofsettings},
by intentionally
changing the default camera parameters to certain sub-optimal settings
denoted by S1, S2, S3 and S4 and measured the Recall for face
recognition AU as before. 
In these settings, the frames from the
camera are of poor quality and we show the Recall for various
thresholds, which is quite low for all the settings. Then, we apply
digital transformation on these using virtual knobs and note the
highest Recall value that we can obtain. 

~\figref{fig:param-tune-vs-postprocess} shows the results.  We see
that for each of the four sub-optimal camera settings, post-processing
improved the Recall compared to the original video, but the Recall is
still quite low.  This is because, due to the sub-optimal camera
settings, the frames from the camera do not have adequate information
about the scene being captured. In contrast, if we directly change the actual
camera parameters, shown as ``Best setting", then we are able to
achieve the highest Recall, \ie 100\%. 
%    Since we already achieve the
%    highest possible Recall value, applying further digital transformation
%    on this will not help any further. 
This result shows that modifying camera
parameters is fundamentally different from applying transformations to
the frames retrieved from the camera.


 \begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_1_excel_1.png}
    \caption{Suboptimal Setting-1 (S1)}
    \label{fig:recall_night_1}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_2_excel_1.png}
    \caption{Suboptimal Setting-2 (S2)}
    \label{fig:recall_night_2}
\end{subfigure}
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_3_excel_1.png}
    \caption{Suboptimal Setting-3 (S3)}
    \label{fig:recall_night_3}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1 in]{figs/recall_night_4_excel_1.png}
    \caption{Suboptimal Setting-4 (S4)}
    \label{fig:recall_night_4}
\end{subfigure}
 \caption{\textit{Parameter Tuning} vs \textit{Postprocessing} for \emph{NIGHT}}
  \label{fig:param-tune-vs-postprocess}
 \vspace{-0.2in}
\end{figure}


\cut{
In summary, 
environmental changes can result in low-quality image acquisition, which in
turn result in poor analytics accuracy. Tuning the camera parameter
settings during capture can provide improvement in accuracy of
AUs, but such camera parameter
tuning is hard for a human to do manually because the best
parameter combination will vary with location of the camera, the type of
analytics units, and the environmental conditions.
%  Humans cannot keep
% adjusting these parameters manually, 
This calls for developing methods 
that can automatically and dynamically tune camera parameters
to improve the accuracy of AUs.
}


% We discuss the challenges and our approach in designing such a system
% design in the next section.


==> oldfiles/related.tex <==
\section{Related Work}

%\subsection{Configuration and tuning of video analytics algorit}
%Recently, tuning knobs after frame-acquisition from the edge-camera (/ISP)-pipeline for better analytics and resource-utilization has gained a lot of attention. 
Several recent proposals have investigated the tuning of parameters of vision algorithms to improve computing resource usage of video analytics pipelines. 
VideoStorm~\cite{201465} tunes parameters of vision algorithms like frames-per-second, frame resolution and internal algorithmic parameters (like the sliding window to search for objects in object detectors, for example) to ensure efficient resource management while processing video analytics queries. However, they do not address tuning of camera parameters. Similarly, Chameleon~\cite{jiang2018chameleon} dynamically picks the best configuration of values for algorithmic parameters like resolution, frame sampling rate, type of detector (e.g., Yolo, VGG or AlexNet) in typical neural-network based video analytics pipelines, based on the video content. However, they also do not address tuning of camera parameters to enhance video analytics. 

%adapts the video pipeline to dynamic video content and reduces the cost of periodic reprofiling by leveraging spatial temporal correlations of configurations [i.e., fps, resolution].
Recent proposals have also considered optimizations to improve network resource usage of video analytics pipelines.
AWStream~\cite{zhang2018awstream} describes methods to make streaming
applications to be adaptive by incorporating the ability to optimally
trade-off accuracy of insights for wide-area network bandwidth consumption. Others
~\cite{234849} have considered sending the video stream in low resolution from the edge to the cloud over a wide-area network, but recover the high-resolution frames from the low-resolution stream via a super-resolution procedure tailored for the actual analytics tasks.
%proposes to tune \textit{frame-skipping}, \textit{bit-rate} and \textit{downsizing} before offloading the frames, then apply analytics-aware expensive super-resolution algorithm to get back the high-resolution frame again before the analytics to be performed on server.
A recent proposal ~\cite{du2020server} also suggests compressing regions of little or no interest more heavily while compressing regions of interest with a lower compression rate to better use the scarce network bandwidth between the sensor and the analytics server. Again, none of these approaches consider dynamic tuning of camera parameters to adapt to changing environmental conditions.
%All these parameter (i.e., fps, resolution) tuning are applied once frames are captured and post-processed by edge-camera. But if continuously inferior-quality frame acquisition is happening due to camera-misconfigurations (i.e., image-appearance knobs in ISP pipeline, brightness, sharpness etc), then network and processing resource will be wasted without any desired analytics being performed. Our approach endeavours to fix these camera-misconfigurations through tuning the image-appearance knobs in the edge-camera depending on external environmental conditions. 
%\subsection{On-camera filtering for better analytics}
%Recently, several research-works are focusing on reducing the offload bandwidth requirement for various analytics in an edge-cloud collaborative scenario without degrading the AU accuracy. 
Focus~\cite{222587} uses a lightweight tiny-yolo model executing on the sensor device to screen frames that are sent for further analytics processing. Others \cite{MLSYS2019_85d8ce59, 10.14778/3137628.3137664} propose binary classifiers to screen frames for analytics processing only when the frames contain the object of interest. The goal here is to reduce the network resource usage. Several techniques ~\cite{chen2015glimpse, li2020reducto} also compare consecutive frames and exploit temporal redundancy in video streams to screen frames that are considered for analytics processing. 
%suggest to offload a frame when it significantly differs from the earlier offloaded frame (i.e., offload when needed) to improve the processing speed of AU pipeline along with reducing the demand for wireless network bandwidth.
In our proposed approach, we use AQuA~\cite{paul2021aqua} to screen poor-quality frames to reduce network bandwidth usage.  However, all these methods do not consider dynamic tuning of camera parameters to enhance the quality of the sensor output. 
%to discard frames on which AU can provide high-confidence error. But alongwith the filtering, our system endeavours to tune the camera-parameters to reduce low-quality processed frame-generation in future during capture, instead of only filtering frames after the capture by existing approaches.



%\subsection{Tunable Video-camera pipeline}
There is a considerable body of work to configure image signal processing pipeline (ISP) in cameras to improve human-perceived quality of images from the cameras. 
%The ISP pipeline is shown in \figref{fig:pipeline}. The goal of these optimizations is to improve human-perceived image quality. 
For example,  VisionISP~\cite{wu2019visionisp} modifies the ISP pipeline to reduce the size of final image output by reducing the bit-depth and resolution. Others have proposed custom optimizations of the ISP for specific computer-vision tasks~\cite{heide2014flexisp, wu2019visionisp, schwartz2018deepisp,  heide2014flexisp, zhang2018ffdnet, liu2020joint, diamond2021dirty, nishimura2019automatic}.
%Traditional camera-pipeline (i.e., ISP pipeline, how camera generates human-readable images from external environment also shown in ~\figref{fig:pipeline}) is primarily optimized to improve human-perceived image-quality. But recently, there has been a consistent effort towards improving the flexibility of this video camera pipeline to make it as custom-tailored for computer-vision tasks~\cite{heide2014flexisp, wu2019visionisp, schwartz2018deepisp}. \cite{heide2014flexisp} replaces the traditional camera-pipeline to a single module putting all other modules' modelled error together. VisionISP~\cite{wu2019visionisp} through modifying the ISP pipeline for machine consumption, can able to reduce the size of final image output by reducing the bit-depth and resolution while preserving relevant information. 
%There also has been significant effort to improve tunability of a specific module in ISP pipeline e.g., demosaicing, denoising, tone-mapping etc. \cite{zhang2018ffdnet} provides faster denoising module for a wide-range of noise levels using a single flexible CNN. Along with denoising, optimizing demosaicing jointly through content-aware self-guidance network helps to reduce the color-artifacts while simultaneously preserving the image-details for better human-perceived image generation~\cite{liu2020joint}. \cite{diamond2021dirty} proposes a end-to-end differentiable architecture for joint denoising, deblurring and classifier to improve classifiers' performance specifically for low-light capture scenario. Since, ISPs are not always differentiable hence, \cite{nishimura2019automatic} proposes a gradient-free nonlinear optimization of tuning ISP pipeline for human perception. 
However, careful re-design or optimization of ISP module for specific vision tasks is time consuming. In our proposed approach, we do not modify the ISP pipeline, and focus on dynamic tuning of configurable camera parameters to consistently produce high-quality sensor output, and enhance the quality of insights from analytics tasks.


%\subsection{Parameter tuning for Human-perceived Quality Improvement}
%There has been an numerous effort for enhancement of final image quality metrics~\cite{ssim,jin2019ilgnet,brisque_mittal2012no,gmlog_xue2014blind,cornia_ye2012unsupervised,Kang_2014_CVPR} perceived by human. In this context, Adobe premier-pro~\cite{adobe-premiere}, adobe lightroom ~\cite{adobe-lightroom} are one of the pioneering industry-leading video-editing tools on captured and processed frame by edge-camera. Recently, super-resolution generative adversarial networks (SR-GANs) attracts researchers' attention through improving image-quality by reducing perceptual loss function~\cite{johnson2016perceptual,yang2014single}.  \cite{jia2021multi} shows the use of particle-swarm optimization to tune parameters of a set of filters for human-perceived image quality enhancement. Authors in ~\cite{dong2017learning} proposed a general method to learn parameter tuning for adaptive image-processing based on local image content. The proposed learning algorithm has shown promising improvement of quality of processed image while applied on classical problems like denoising, demosaicing and deblurring. 

%add super-resolution and adobe-premier pro

%robustness of object-detection based on deep-learning models, objectRL,

==> oldfiles/vc.tex <==
\section{Virtual camera}
\label{sec:vc-sim}
\begin{figure}[b]
 \centering
    \includegraphics[width=0.99\linewidth]{figs/evaluation-setup.png}
    \caption{$\approach$ system design with VC}
    \label{fig:eval_setup}
\end{figure}

%discuss the pipeline first same as figure 9
%then why we want to abstract physical camera pipeline to virtual camera
%put the benefits of VC on the top to motivate the section
%faster training scalable for 100 of cameras


\subsubsection{Need}
RL module, described in Section \ref{camera-parameters-tuning}, requires the agent to \textit{learn} by going through different \textit{states}, taking different \textit{actions} and correctly interpreting the corresponding \textit{reward}. This learning process requires that the video feed goes through various environmental changes, so that the model developed is robust. If we work with real cameras, it may take weeks or even months to go through such changes. It is not practical to wait so long to train the model. Besides, it does not give the flexibility to test various reward functions because the conditions are not reproducible and experiments are not repeatable in such a setup. Therefore, we propose a virtual camera (VC), which mimics a real camera, but it does not have the drawbacks of working with a real camera to train the RL module. VC allows us to (a) conduct experiments where various camera parameter configurations can be applied to the exact same scene, which enables us to have repeatability and reproducibility in our experiments (note that this is not possible with a real camera), (b) run the experiments much faster than real-time; we can process video frames at a much higher frame rate like 300 frames per second rather than the 25-30 frames per second from a real camera, and (c) independently test and train RL algorithms with various reward functions. Along with these, in scenarios where there are multiple AUs running on a single video feed, it may happen that each AU requires a different ``best" camera setting. However, it is not possible to have separate camera settings for each AU, since there can be only one camera setting at any given point in time. In such scenarios, VC can be used by each AU and custom ``best" camera setting can be simulated through VC as per specific AU requirements ~\cite{jang2018application}.

%\textcolor{blue}{
%Along with these three main benefits, VC also enables different AUs to have their own custom best parameter setting while multiple AUs are running on same video feed to have insights and each AU requires a different camera parameter setting~\cite{jang2018application}. 
%}
\if 0
%\textcolor{red}{why vc needed?} \\
%-->Difficult to evaluate the pipeline, if we can't tryout different configurations on same content and scene-characteristics. There won't be any repeatability or reproducibility. 

%--> VC approach also helps to train the RL algorithm faster, aids RL algorithm developement. Not only different configurations or actions but also different reward functions can be tried.

%In order to study the effectiveness of $\approach$, one approach is to work with real cameras and show the impact of our approach by comparing the AU accuracy in two cases i.e. first case where we don't apply our technique and have static camera parameters, and in the second case, we apply our technique and dynamically tune camera parameters. But, the problem with this approach is that the camera can have only one set of parameters at any given point in time and we cannot run both conditions (with and without our technique) at the same time using a single camera. If we think of doing it at separate times, then the environmental (e.g. sunny, cloudy, etc.) as well as the scene conditions (e.g. faces seen in the field of view) will be different, and therefore, it will not be a fair comparison.

%An alternate approach is to use two cameras, where we run the AU on one camera feed and keep the camera parameters fixed, while the on the other camera feed we run the same AU but we dynamically tune the camera parameters. After the two experiments, we can compare the measured accuracy of insights. In this scenario the environmental conditions seen by the two cameras will be similar, however the scene conditions, although similar, won't be exact due to displacement of the two cameras. 
%The issue is that the view point and angle of the two cameras is not identical, due to which, the accuracy of AU may vary. For example, even with a slight variation in the angle of the face being observed, the face detection AU can give different result. 
%Some AUs can be very sensitive and may not give same result on similar images i.e. result depends on very fine characteristics in the frame and may produce different results with slight variations in image. Therefore, even this will not be a fair comparison. Besides, even if the AU is tolerant to slight variations in images, since the changes in environmental conditions is not deterministic, it will take very long to perform various experiments, including trying out different configurations, training and testing RL algorithms, trying different reward functions for RL, etc.

%Because of the problems discussed above in using real camera feeds, we decided to study the effectiveness of our approach by using pre-recorded videos. These videos are recorded with a single camera setting in broad daylight condition. By doing so, we have good quality original video feed which has certain environmental conditions (daylight, in this case) and certain scene conditions (e.g. faces of people), and we can also obtain the ground truth on these videos. We then simulate two cameras, which we call as virtual cameras, such that they expose same parameters as real cameras and we can change these parameters through APIs. By doing so, we are able to (a) Conduct experiments with various configurations being applied to exact same scene, which enables us to have repeatability and reproducibility in our experiments, which is not possible with a real camera and (b) We can run the experiments faster than real-time i.e. run through frames at a higher FPS, as desired, and be able to independently test and train RL algorithms with various reward functions used for RL, etc.

\fi

\subsubsection{Design}
In order to mimic a real camera, VC accepts a pre-recorded video and the time of the day as input. Based on the time of the day and current VC camera parameters, which we refer to as virtual knobs, VC applys transformation on the frames and produces the final image. Note that VC exposes APIs, similar to a real camera, to change the virtual knobs. Fig. \ref{fig:eval_setup} shows $\approach$ system design with VC, where the RL agent changes the virtual knobs and learns much quickly using such a setup with VC. VC design consists of two phases: (a) offline profiling phase, (b) online phase.

%Due to the issues explained in ~\secref{sec:eval-method} regarding either using two different closely located camera feeds or same camera feed at different times, we have to loop the same original pre-recorded video through two virtual cameras. 
%These virtual cameras need to emulate the same daylong environmental variation starting from sunrise, to noon, afternoon, dusk, night etc. ~\figref{fig:eval_setup} shows the control loop to modify virtual camera parameters (a.k.a virtual knobs) which apply different transformations based on the time of the day, enables same scene to adapt different environmental conditions. 
%VC simulator design consists of two phases: (a) offline profiling phase, (b) online phase.




\begin{algorithm}[t]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwFunction{FExtract}{ExtractFeatures}
  \SetKwFunction{FDecode}{DecodeFrames}
  \SetKwFunction{FSplit}{SplitFrame}
  
  \caption{VC Table Generation}
  \label{alg:vc}
  \Input{\begin{minipage}[t]{6.5cm}%
     5-minute video-snippets $V_S$;
   \end{minipage}
  }
\tcp{divide 24 hours into 96 equal intervals, each being 15 min long ($intvl$)}
\For{index in range(0,96)}{
    \For{$V_S$ with capture-timestamp $\in$ $intvl_{index}$}
    {
        frames $\leftarrow$ \FDecode($V_S$)\\
        \For{frame $in$ frames}{
            \tcp{split each frame into 12 tiles}
            tiles $\leftarrow$ \FSplit(frame)\\
            \tcp{featureTuple$\leftarrow$<brightness,contrast,color,sharpness>}
            \For{tile $in$ tiles}{
               featureTuple$_{tile}$ = \FExtract(tile)
            }
        }
    }
    \tcp{compute mean feature values across all videos captured with 15 min}
    Compute Mean Value featureTuple$_{tile}^{intvl}$ 

}
\KwRet{12 tables storing Mean featureTuple$_{tile}^{intvl}$ corresponding to each tile for each 15 minute interval}
}

\end{algorithm}



\begin{algorithm}[t]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwFunction{FExtract}{ExtractFeatures}
  \SetKwFunction{FDecode}{DecodeFrames}
  \SetKwFunction{FAug}{RenderFrame}
  
  \caption{Delta-change to Configuration mapping Table Generation}
  \label{alg:delta-config}
  \Input{\begin{minipage}[t]{6.5cm}%
     5-minute video-snippets $V_S$; $r_B, r_{Con}, r_{Col}, r_S$ are virtual knob ranges obtained from ~\tabref{tab:cam-twin-final};
   \end{minipage}
  }
\tcp{each 15 min interval, $intvl$}
  \For{randomly selected $Frame$ from each interval}{
  \For{tile in range(1,13)}{
    \tcp{featureTuple$\leftarrow$<brightness,contrast,color,sharpness>}
    featureTuple$_{tile}^{org}$ $\leftarrow$ \FExtract($frame_{tile}$) \\
    \For{$virtual_{conf}$ $\in$ ($r_B$$\circ$$r_{Con}$$\circ$$r_{Col}$$\circ$$r_S$)}
    {
            \tcp{<Bright, Contrast, Color, Sharp> $\leftarrow$ $virtual_{conf}$}
            $virtFrame_{tile}$ $\leftarrow$ \FAug($Frame_{tile}$, $virtual_{conf}$)\\
            $featureTuple_{tile}^{virt}$ $\leftarrow$ \FExtract($virtFrame_{tile}$)\\
            \tcp{compute delta changes after re-rendering}
            delta[0] = $\frac{featureTuple_{tile}^{virt}[0]}{featureTuple_{tile}^{org}[0]}$\\
            compute delta[1], delta[2], delta[3] for 3 other knobs \\
            Store <delta> corresponding to $virtual_{conf}$\\
        }
    }
  }
Compute Median <delta> for same $virtual_{conf}$ across sampled frames for a specific tile \\
\KwRet{12 <delta>-vs-configuration Mapping tables for each tile}\\
}
\end{algorithm}

\begin{algorithm}[t]
{ 
\small
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwFunction{FExtract}{ExtractFeatures}
  \SetKwFunction{FDecode}{DecodeFrames}
  \SetKwFunction{FAug}{RenderFrame}
  \SetKwFunction{FSplit}{SplitFrame}
  \SetKwFunction{FCM}{FindClosestMap}
   \SetKwFunction{FGM}{GetMedian}
  
  \caption{Runtime VC Simulator}
  \label{alg:vc-sim}
  \Input{\begin{minipage}[t]{6.5cm}%
  input frame corresponding to time $T1$, inpFrame$^{T1}$;
  Output Time $T2$;
   \end{minipage}
  }
  
  \Output{\begin{minipage}[t]{6.5cm}%
  input frame corresponding to output time $T2$, inpFrame$^{T2}$;
   \end{minipage}
  }

  \tcp{split input frame into 12 tiles}
  inpFrame$_{tile}^{T1}$ $\leftarrow$ \FSplit(inpFrame$^{T1}$)\\
  \For{tile in range(1,13)}{
  \tcp{featureTuple$\leftarrow$<brightness,contrast,color,sharpness>}
  \tcp{Measure input frame features}
  featureTuple$_{tile}^{T1}$ $\leftarrow$ \FExtract(inpFrame$_{tile}^{T1}$)\\
  \tcp{obtain features corresponding to output time}
  Get featureTuple$_{tile}^{T2}$ from VC-table ~\ref{alg:vc}\\
  \tcp{compute delta change from T1 to T2 for 4 knobs}
  delta[0] = $\frac{featureTuple_{tile}^{T2}[0]}{featureTuple_{tile}^{T1}[0]}$\\
  Similarly obtain delta[1], delta[2] and delta[3] \\
  config $\leftarrow$ \FCM(<delta>) using L1 norm distance and table generated in Alg~\ref{alg:delta-config}\\
  append config to a configList\\
  }
  config$_{median}$ $\leftarrow$ \FGM(configList)\\
  inpFrame$^{T2}$ $\leftarrow$ \FAug(inpFrame$^{T1}$, config$_{median}$)
}
\end{algorithm}

%During \textit{offline profiling phase}, first, following algorithm~\ref{alg:vc}, we generate VC table, \textit{a mapping function that maps a particular time in a day to its corresponding <brightness, contrast, color-saturation, sharpness> feature values observed during that time.} As different parts of the frame may have different characteristics e.g. due to presence of obstacle, shadows, different lighting, etc., instead of computing these feature values for the entire frame, we divide the frame into 12 tiles and obtain the feature-values for each tile, as shown in \figref{fig:vc-tiles}. \figref{fig:vc-profile} shows how different tiles exhibit different brightness, contrast, color-saturation and sharpness profile across different hours of the day. 

\textbf{Offline profiling phase}: This phase consists of two parts. \textit{First}, to obtain a mapping between time of the day and the corresponding feature tuple (consisting of brightness, contrast, color-saturation and sharpness values) for that time. \textit{Second}, to obtain a mapping between delta change between two feature tuples and the corresponding virtual knob value. These mapping tables are used in \textit{online} phase to render the frame by VC.

Algorithm~\ref{alg:vc} shows the procedure to obtain the mapping between time of the day and corresponding feature tuple. We refer to this mapping as VC table. To generate this VC table, we use a full 24 hour long video which is broken into 5 minute video snippets. The VC table that we generate has a granularity of 15 minutes i.e. for a period of 15 minutes, we have a corresponding feature tuple. Thus, we have total 96 intervals in a 24 hour period and for each interval, we have 3 video snippets. We go through each of these video snippets, extract the frames, and for each of the frames, we divide the frame into 12 tiles (to account for variation in local feature values in different parts of the frame, as shown in ~\figref{fig:vc-tiles}), and for each tile, we obtain the corresponding feature tuple (variation of these different features across entire day for each tiles is shown in ~\figref{fig:vc-profile}). We then compute the mean for each tile for a 15 minute interval. This forms the VC table, with feature tuple values for each tile for each 15 minute interval, as shown in~\figref{fig:vc-table}.

Algorithm~\ref{alg:delta-config} shows the procedure to obtain the mapping between delta change between two feature tuples and the corresponding virtual knob value. As in Algorithm~\ref{alg:vc}, we use a full 24 hour long video which is broken into 5 minute video snippets. As before, we use a granularity of 15 minutes as our interval and select a random frame within an interval to form a collection of frames with varying conditions. Again, for each of these frames, we consider separate tiles (total 12) and for each of the tile, we extract the feature tuple (original). Now, using the ranges obtained from Table \ref{tab:cam-twin-final}, we generate all combinations of the possible virtual configurations, and for each of those configurations - we render the frame using the specific virtual configuration, extract the feature tuple on the rendered frame and then compute the delta change between the original and rendered frame for each of the feature tuple. This forms a mapping between the delta change and the corresponding virtual configuration. Now, we have such mapping for each of the randomly selected frames and for each tile. Lastly, we combine the delta values across all frames by taking the median and generate a table, called VC delta-change table, consisting of mapping between the delta change and corresponding virtual configuration value, for each tile, as shown in~\figref{fig:delta-to-config}.

%Each pre-recorded video captures the content as well as the environment for that particular acquisition-time. Since, we need to keep the observed content same by VC, only environmental condition throughout the day affects the captured frame. Through camera-parameter tuning RL approach (shown in ~\figref{fig:system_design}, we endeavour to minimize the adverse environmental affect on AU performance. Keeping the content same,  to augment the video for different time of the day, we need to generate another mapping table that maps the <brightness, contrast, color-saturation, sharpness> change between two times to corresponding virtual camera knob configuration to achieve that change. In offline phase, we generate this \textit{delta change-to-Configuration mapping table} following the algorithm~\ref{alg:delta-config}.

%Each pre-recorded video captures the content as well as the environment for that particular acquisition-time. With VC the actual content in the frame remains the same, however the rendering of the frame can be changed by tuning virtual knobs. With RL (shown in ~\figref{fig:system_design}), we endeavour to minimize the adverse environmental affect on AU performance by rendering the frame in a better manner. Keeping the content same, to render the video for different times of the day, we need to generate another mapping table that maps the <brightness, contrast, color-saturation, sharpness> change between two times to corresponding VC knob configuration to achieve that change. In offline phase, we generate this \textit{delta change-to-Configuration mapping table} following the algorithm~\ref{alg:delta-config}.

%During \textit{online phase}, to simulate a frame for a different environmental condition corresponding to a time of the day other than its capture time, following the algorithm~\ref{alg:vc-sim}, we first split the input frame into 12 tiles as shown in~\figref{fig:vc-tiles}. Now for each tile, we need to extract the 4 different feature values, and also based on the desired time (other than capture time) and using the VC table (i.e., output of algorithm~\ref{alg:vc}, we can get the tile-specific desired values of the image features. The fractional delta-change between the current feature values and desired feature values will be mapped to a virtual camera knob configuration value using delta change-to-Configuration mapping table (i.e. output of algorithm~\ref{alg:delta-config}). 
%Although, we obtain different knob configurations for each tile, but in order to eliminate the \emph{tiling-issue} (i.e., separation of tiles is explicit) in the output frame, we compute the median configuration across all 12 configurations corresponding to each tile. With the modified median knob configuration, we can get the video-frame for the desired time. 
\textbf{Online phase}: During \textit{online phase}, VC actually transforms the pre-recorded input video (of time $T1$) to any other desired time of the day ($T2$), provided as input. Algorithm~\ref{alg:vc-sim} shows the procedure followed by VC to perform this transformation. Each input frame of time $T1$ is first split into 12 tiles. Then, for each tile, feature tuple is extracted. Then, for the desired time $T2$, the corresponding feature tuple is obtained from VC table (output from algorithm~\ref{alg:vc}). Delta change between the feature tuple at time $T2$ and time $T1$ is then computed. The virtual configuration values corresponding to the closest delta change (using L1 norm distance~\cite{l1}) is obtained from VC delta-change table (output from algorithm~\ref{alg:delta-config}). Once the configuration is obtained for each tile, a median configuration is computed across tiles (to eliminate visibility of distinct tiles in the frame) and this configuration is used to render the frame for time $T2$. Thus, the frame at time $T1$ is transformed by VC to a frame at time $T2$.

While training the RL module, as shown in~\figref{fig:eval_setup}, RL agent uses the APIs exposed by VC to change the virtual knob values and learns much quickly, as (a) different environmental conditions can be generated easily by VC (b) frames can be processed at a much faster rate, even up to 300 FPS, by using more computing hardware, and (c) virtual knob values can be changed instantly.

\begin{figure}[t]
 \centering
    \includegraphics[width=0.7\linewidth]{figs/vc-tiles.png}
    \caption{Tiled representation of a captured frame}
    \label{fig:vc-tiles}
\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/vc-tiles.PNG}
    %\vspace{-0.2in}
%    \caption{Tiled representation of a captured frame}
%    \label{fig:vc-tiles}
    %\vspace{-0.1in}
%\end{figure}


 \begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_bright_part_1.pdf}
    \caption{Brightness}
    \label{fig:vc-bright}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_contrast_part_1.pdf}
    \caption{Contrast}
    \label{fig:vc-contrast}
\end{subfigure}
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_color_part_1.pdf}
    \caption{Color-Saturation}
    \label{fig:vc-color}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=1.2 in]{figs/8_sharp_part_1.pdf}
    \caption{Sharpness}
    \label{fig:vc-sharp}
\end{subfigure}
 \caption{Day-long feature profiles for different tiles}
  \label{fig:vc-profile}
 %\vspace{-0.2in}
\end{figure}


\if 0
\begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[Brightness]{\includegraphics[width=3.8cm]{figs/8_bright_part_1.pdf}\label{fig:vc-bright}}
 & \subfloat[Contrast]{\includegraphics[width=3.8cm]{figs/8_contrast_part_1.pdf}\label{fig:vc-contrast}
 } \\
 
 \subfloat[Color-Saturation]{\includegraphics[width=3.8cm]{figs/8_color_part_1.pdf}\label{fig:vc-color}}
 & \subfloat[Sharpness]{\includegraphics[width=3.8cm]{figs/8_sharp_part_1.pdf}\label{fig:vc-sharp}
 } \\
 \end{tabular}
 \end{tabularx}
 \caption{Day-long feature profiles for different tiles}
  \label{fig:vc-profile}
   %\vspace{-0.2in}
 \end{figure}
 \fi
 
 
 \begin{figure}[tb]
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=0.6 in]{figs/vc-table.PNG}
    \caption{VC Table}
    \label{fig:vc-table}
\end{subfigure}%
\begin{subfigure}[]{0.5\linewidth}
\centering
    \includegraphics[height=0.6 in]{figs/delta-table.PNG}
    \caption{Delta-to-Configs Table}
    \label{fig:delta-to-config}
\end{subfigure}
 \caption{Offline Generated Tables}
  \label{fig:vc-tables}
 %\vspace{-0.2in}
\end{figure}
 
 
 \if 0
 \begin{figure}
\def\tabularxcolumn#1{m{#1}}
 \begin{tabularx}{\linewidth}{@{}cXX@{}}
 \begin{tabular}{cc}
 \subfloat[VC Table]{\includegraphics[width=3.8cm]{figs/vc-table.PNG}\label{fig:vc-table}}
 & \subfloat[Delta-to-Configs Table]{\includegraphics[width=3.8cm]{figs/delta-table.PNG}\label{fig:delta-to-config}
 } \\
 \end{tabular}
 \end{tabularx}
 \caption{Offline Generated Tables}
  \label{fig:vc-tables}
   \vspace{-0.2in}
 \end{figure}
\fi 
 

 
 





























\if 0
 \begin{table}[h!]
 \parbox{.35\linewidth}{
\centering
 \begin{tabular}{|c|c|}
\hline
time & feature-values \\ \hline
10:00 & <159,53,11,2122> \\ \hline
10:15 & <160,52,13,2100> \\ \hline
... & ... \\ \hline
\end{tabular}
\caption{VC Table}
}
\hfill
\parbox{.35\linewidth}{
 \begin{tabular}{|c|c|}
\hline
delta change & configurations \\ \hline
<0.5,0.7,1.5, 2> & <0.7,0.6,1.1,1..2> \\ \hline
<19,24,45,9> & <1.6,2.4,1.6,1.5> \\ \hline
... & ... \\ \hline
\end{tabular}
\caption{delta-change to configuration mapping}
}
\label{tab:best-video-conf}
 %\vspace{-0.3in}
\end{table}
\fi
